Graph Neural Networks: Architectures, Stability and Transferability

Graph Neural Networks (GNNs) are information processing architectures for signals supported on graphs. They are presented here as generalizations of convolutional neural networks (CNNs) in which individual layers contain banks of graph convolutional filters instead of banks of classical convolutional filters. Otherwise, GNNs operate as CNNs. Filters are composed with pointwise nonlinearities and stacked in layers. It is shown that GNN architectures exhibit equivariance to permutation and stability to graph deformations. These properties help explain the good performance of GNNs that can be observed empirically. It is also shown that if graphs converge to a limit object, a graphon, GNNs converge to a corresponding limit object, a graphon neural network. This convergence justifies the transferability of GNNs across networks with different number of nodes. Concepts are illustrated by the application of GNNs to recommendation systems, decentralized collaborative control, and wireless communication networks.

==> ch8_sec02_permutation_invariance_filters.tex <==
% !TEX root = ../compile_all_book/gsp.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Permutation Equivariance of Convolutional Graph Filters}\label{sec_ch8_permutation_invariance_filters}

The learning parametrization in \eqref{eqn_ch8__erm_graph_filter} utilizes convolutional graph filters. We recall from our discussion in \red{Chapter \ref{ch_filters}} that these are given by matrices of the form $\bbH(\bbS) := \sum_{k=0}^{\infty} h_{k} \bbS^{k}$ which, for an input graph signal $\bbx$, produce the output graph signal
% 
\begin{equation} \label{eqn:graphFilter}
	\bbz \  = \ \sum_{k=0}^{\infty} h_{k} \bbS^{k} \bbx
	     \ := \ \bbH(\bbS) \bbx .
\end{equation}
%
The output $\bbz$ resulting from application of the shift invariant graph filter to the graph signal $\bbx$ is another graph signal supported on the same graph. Such output depends on the input signal $\bbx$ and the filter coefficients $\bbh$ as well as on the graph shift operator $\bbS$. We have generically thought of graph filters as a specific set of coefficients applied on a specific graph. In this section we think of a filter as being defined by the set of coefficients $\bbh$ which we can run on any given graph. For reference, if we are given a shift operator $\hbS$ we can define the filter $\bbH(\hbS):=\sum_{k=0}^{\infty} h_{k} \hbS^{k}$ whose application to signals $\hbx$ produces signals
% 
\begin{equation} \label{eqn:graphFilter_perturbed}
	\hbz \  = \ \sum_{k=0}^{\infty} h_{k} \hbS^{k} \hbx
	     \ := \ \bbH(\hbS) \hbx .
\end{equation}
%
We want to study the relationship between $\bbH(\bbS)$ and $\bbH(\hbS)$ when $\bbS$ and $\hbS$ are permutations of each other. Formally, given a dimension $N$ we define permutation matrices $\bbP$ as those that belong to the set
%
\begin{equation} \label{eqn:permutationSet}
    \ccalP = \left\{
        \bbP \in \{0,1\}^{N \times N}
            :
        \bbP \bbone = \bbone , 
        \bbP^{\Tr} \bbone = \bbone
    \right\}.
\end{equation}
%
As per \eqref{eqn:permutationSet}, a permutation matrix $\bbP$ is one in which the product $\hbx = \bbP\bbx$ is a reordering of the entries of the vector $\bbx$. Likewise, for a given shift operator $\bbS$, the shift operator $\hbS = \bbP^{\Tr}\bbS\bbP$ is a reordering of the rows and columns of $\bbS$. Thus, the graph $\hbS$ is just a relabeling of the nodes of $\bbS$. Taken together, the graph $\hbS = \bbP^{\Tr}\bbS\bbP$ and the signal $\hbx = \bbP\bbx$ represent a consistent relabeling of the graph $\bbS$ and the graph signal $\bbx$. One would expect that application of the filter on the relabeled graph to the relabeled signal produces and output that corresponds to the relabeled output prior to permutation of the graph. The following proposition asserts that this is true.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   P   R   O   P   O   S   I  T   I   O   N   %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{proposition}[Permutation equivariance] \label{prop_ch8_filterPermutationEquivariance} Consider graph shifts $\bbS$ and $\hbS = \bbP^{\Tr} \bbS \bbP$ for some permutation matrix $\bbP \in \ccalP$ [cf. \eqref{eqn:permutationSet}]. Given a set of coefficients $\bbh$, the filters $\bbH(\bbS)$ and  $\bbH(\hbS)$ in \eqref{eqn:graphFilter} and \eqref{eqn:graphFilter_perturbed} are such that for any pair of corresponding graph signals $\bbx$ and $\hbx = \bbP^{\Tr}\bbx$ the graph filter outputs $\bbz := \bbH(\bbS) \bbx $ and $\hbz := \bbH(\hbS) \hbx $
% 
\begin{equation}\label{eqn_ch8_prop_filter_permutation_equivariance}
   \hbz \, := \, \bbH(\hbS) \hbx
        \, := \, \bbH(\hbS) \Big( \bbP^{\Tr}\bbx \Big) 
        \, =  \, \bbP^{\Tr} \Big(  \bbH(\bbS) \bbx \Big)
        \, := \, \bbP^{\Tr} \bbz.
\end{equation} \end{proposition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   P   R   O   O   F   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{proof} Being a permutation matrix, $\bbP$ is an orthogonal matrix. Thus $\bbP^{\Tr} \bbP = \bbP \bbP^{\Tr} = \bbI$ from where it follows that powers $\hbS^k$ of a permuted shift operator are permutations of the respective shift operator powers $\bbS^k$
% eqn
\begin{equation}\label{eqn_ch8_prop_equivariance_pf_10}
    \hbS^{k} = (\bbP^{\Tr} \bbS \bbP)^k
             = \bbP^{\Tr} \bbS^{k} \bbP.
\end{equation}
%
Substituting this fact in the definition of the permuted graph filter $\bbH(\hbS)$ in \eqref{eqn:graphFilter_perturbed} yields
% eqn
\begin{equation}\label{eqn_ch8_prop_equivariance_pf_20}
    \bbH(\hbS) 
%        = \sum_{k=0}^{\infty} h_{k} \hbS^{k} 
        = \sum_{k=0} h_{k} \left( \bbP^{\Tr} \bbS^{k} \bbP \right) 
        =  \bbP^{\Tr}\bigg( \sum_{k=0} h_{k}  \bbS^{k}  \bigg) \bbP.
\end{equation}
%
In the last equality the sum is the filter $\bbH(\bbS) = \sum_{k=0} h_{k}  \bbS^{k}$ as defined in \eqref{eqn:graphFilter}. We can then write $\bbH(\hbS) = \bbP^{\Tr} \bbH(\bbS) \bbP$ and use this fact to express application of the permuted filter $\bbH(\hbS)$ to the permuted signal $\bbP^{\Tr} \bbx$ as
% eqn
\begin{equation}\label{eqn_ch8_prop_equivariance_pf_30}
    \bbH(\hbS) \bbP^{\Tr} \bbx
        = \bbP^{\Tr} \bbH(\bbS) \bbP \bbP^{\Tr} \bbx
\end{equation}
%
Given that the permutation matrix $\bbP$ is orthogonal, as already argued, we have that $\bbP \bbP^{\Tr}=\bbI$. Substituting this into the right hand side of \eqref{eqn_ch8_prop_equivariance_pf_30}, the result in \eqref{eqn_ch8_prop_filter_permutation_equivariance} follows. \end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Proposition \ref{prop_ch8_filterPermutationEquivariance} states the permutation equivariance of graph filters. Namely, a permutation of the input -- from $\bbx$ to $\hbx = \bbP^{\Tr}\bbx$ -- along with a permutation of the shift operator -- from $\bbS$ to $\hbS = \bbP^{\Tr} \bbS \bbP$ -- results in a permutation of the output -- from $\bbz$ to $\hbz = \bbP^{\Tr} \bbz$. Notice that if we are given vectors $\bbx$ and $\hbx = \bbP^{\Tr}\bbx$ and we know the permutation matrix $\bbP$ it is elementary to design linear operators that are permutation equivariant by simply applying the permutation to the linear operator. The permutation equivariance in \eqref{eqn_ch8_prop_filter_permutation_equivariance} is more subtle in that it holds without having access to the permutation $\bbP$. 

The permutation equivariance of graph filters implies that they are useful when considering applications where graph relabelings are inconsequential. This motivates consideration of the space of linear operators modulo permutation along with operator distances between these equivalence classes which we introduce next.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   D   E   F   I   N   I  T   I   O   N   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{definition}[Perturbation Modulo Permutation] \label{def_ch8_operator_distance} 
Given linear operators $\bbA$ and $\hbA$ we define the operator distance modulo permutation as
%
\begin{align} \label{eqn_ch8_def_ch8_operator_distance}
   \big\| \bbA - \hbA \big\|_{\ccalP} 
      \ = \   \min_{\bbP\in\ccalP} \,
                 \max_{ \bbx : \| \bbx \| = 1 } \,
                     \big\|\bbP^{\Tr}(\bbA \bbx)  - \hbA (\bbP^{\Tr} \bbx)\big\| .
\end{align}
%
We denote as $\bbP_0$ a matrix that attains the minimum in \eqref{eqn_ch8_def_ch8_operator_distance} and define the perturbation modulo permutation as the matrix 
%
\begin{align} \label{eqn_ch8_def_ch8_operator_distance_error_matrix}
   \bbE = \bbA - \bbP_0\hbA\bbP_0^T.
\end{align} \end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The distance in \eqref{eqn_ch8_def_ch8_operator_distance} compares the effect of applying the operators $\bbA$ and $\hbA$ to a vector $\bbx$ with a permutation $\bbP$ applied before or after application of the linear operators. It measures this difference at the unit norm vector for which it is largest and at the permutation matrix that makes it smallest. The perturbation matrix $\bbE$ is the difference between operators $\bbA$ and $\bbP_0\hbA\bbP_0^T$ for the permutation matrix $\bbP_0$ that achieves the minimum norm difference in \eqref{eqn_ch8_def_ch8_operator_distance}. If there is more than one matrix that achieves the minimum, an arbitrary choice is acceptable for the results we will derive to hold. Further notice that it follows from \eqref{eqn_ch8_def_ch8_operator_distance} and \eqref{eqn_ch8_def_ch8_operator_distance_error_matrix} that the operator distance between $\bbA$ and $\hbA$ is simply the operator norm of the error matrix $\bbE$,
%
\begin{align} \label{eqn_ch8_def_ch8_operator_distance_error_matrix}
   \big\| \bbA - \hbA \big\|_{\ccalP}  = \| \bbE \|.
\end{align}
%
It is ready to see that Definition \ref{def_ch8_operator_distance} is a proper distance in the space of linear operators modulo permutation. In particular, it holds that $\big\| \bbA - \hbA \big\|_{\ccalP} = 0$ if and only there exists a permutation matrix for which $\hbA = \bbP^T \bbA \bbP$. From this latter fact it follows that we can rewrite Proposition \ref{prop_ch8_filterPermutationEquivariance} to say that the distance modulo permutation between graph filters $\bbH(\bbS)$ and $\bbH(\hbS)$ is null if the distance modulo permutation between the shift operators  $\bbS$ and $\hbS$ is null. We formally state and prove this fact in the following corollary.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   C   O   R   O   L   L   A   R   Y   %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{corollary}[Permutation equivariance] \label{prop_ch8_permutation_equivariance} 
For shift operators $\bbS$ and $\hbS$ whose distance modulo permutation is $\| \bbS - \hbS \|_{\ccalP} = 0$, the distance modulo permutation between graph filters $\bbH(\bbS)$ and $\bbH(\hbS)$ satisfies 
%
\begin{equation}\label{eqn_ch8_prop_ch8_permutation_equivariance} 
   \| \bbH(\bbS) - \bbH(\hbS) \|_{\ccalP} = 0.
\end{equation} \end{corollary}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   P   R   O   O   F   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{proof} If $\| \bbS - \hbS \|_{\ccalP} = 0$ there exists permutation $\bbP$ such that $\hbS = \bbP^{\Tr} \bbS \bbP$ and Proposition \ref{prop_ch8_filterPermutationEquivariance} holds. Thus, for this same permutation we have $\bbP^{\Tr}(\bbH(\bbS) \bbx)  = \bbH(\hbS) (\bbP^{\Tr} \bbx)$ for any vector $\bbx$. The result in \eqref{eqn_ch8_prop_ch8_permutation_equivariance} then follows from Definition  \ref{def_ch8_operator_distance}.\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Corollary \ref{prop_ch8_permutation_equivariance} says that if two graphs are the same, the graph filters are also the same, modulo permutation. 

Permutation equivariance is important to establish that the outputs of graph filters are essentially the same regardless of labeling. Permutation equivariance is of further importance in learning contexts because it implies that graph filters exploit the internal symmetries of the graph as we explain next.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t] 
\def\myfactor{0.70}
\centering
\begin{minipage}{0.47\linewidth}\centering
\input{../ch8_gnn/figures/hexagon_graph_signal_node_3_b} %\\ {\small (a)}
\end{minipage} \quad
\begin{minipage}{0.47\linewidth}\centering
\input{../ch8_gnn/figures/hexagon_graph_signal_node_3_c} %\\ {\small (a)}
\end{minipage} 
\caption{Generalization of linear transformations. We expect to be able to classify the right from seeing the left.}
\label{fig_ch8_reco_system_easy_generalization}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\subsection{Equivariance and Graph Signal Symmetries}\label{sec_ch8_equivariance_and_symmetries}

In Section \ref{sec_ch8_reco_systems_stylized} we considered learning product ratings on a graph of user preference similarities. We did so with an arbitrary linear transformation $\Phi(\bbx;\bbH)$ [cf. \eqref{eqn_ch8__reco_system_training_set_arbitrary_linear}] and a graph filter $\Phi(\bbx;\bbh, \bbS)$ [cf. \eqref{eqn_ch8__reco_system_training_set_graph_filter}]. We observed that the graph filter worked better as it attains a smaller mean squared error during testing. Proposition \ref{prop_ch8_filterPermutationEquivariance}, or, equivalently, Corollary \ref{prop_ch8_permutation_equivariance}, show that this is because the graph filter generalizes to examples that have not been seen before in a manner that is impossible for arbitrary linear transformations.  

To explain this point suppose, for the sake of argument, that we train $\Phi(\bbx;\bbH)$ and $\Phi(\bbx;\bbh, \bbS)$ on the input in Figure \ref{fig_ch8_reco_system_example_signals}-right. If a product $p'$ is such that the ratings of users 2, 4, 8, 9, and 10 are similar to their ratings of product $p$, we expect both, $\Phi(\bbx;\bbH)$ and $\Phi(\bbx;\bbh, \bbS)$ to make accurate predictions of the rating user 3 would give to $p'$. Consider now a product $p'$ as in the left pane of Figure \ref{fig_ch8_reco_system_easy_generalization} in which ratings of users 2, 4, 8, 9, and 10 are overall smaller than their ratings of product $p$ but share the same structure -- users 2, 4, and 9 give a betters score than users 8 and 10. We expect again that both, $\Phi(\bbx;\bbH)$ and $\Phi(\bbx;\bbh, \bbS)$ make accurate predictions of the rating of user 3. We can summarize this observation by saying that from the observations in Figure \ref{fig_ch8_reco_system_example_signals} we have learnt to predict for the input signal in the left of Figure \ref{fig_ch8_reco_system_easy_generalization} without having ever observed this signal.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t] 
\def\myfactor{0.70}
\centering
\begin{minipage}{0.47\linewidth}\centering
\input{../ch8_gnn/figures/hexagon_graph_signal_node_3_b_permutation}  %\\ {\small (b)}
\end{minipage} \quad
\begin{minipage}{0.47\linewidth}\centering
\input{../ch8_gnn/figures/hexagon_graph_signal_node_6}  %\\ {\small (b)}
\end{minipage} 
\caption{\red{Permutation equivariance of graph filters. The output of a graph filter is equivariant to graph permutations (Proposition \ref{prop_ch8_filterPermutationEquivariance}). This not only means independence from labeling --left and middle are equivalent-- but it also shows that graph filters exploit internal signal symmetries. The signals on left and right are different signals on the same graph but they are permutations of each other --interchange inner and outer hexagons and rotate $180^\circ$ to obtain middle, which is equal to left. A graph filter would output the same signal whether it processes any of these signals. This has important implications when \emph{learning} the filter coefficients, since how to process the signal in the right can be inferred from seeing examples of the signal in the left. Integer node labels ranging from 1 to 12. Signal values are represented by different colors.} \blue{Rewrite. Shorten and adapt.}}
\label{fig_ch8_reco_system_linear_vs_graph_filter}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   M   A   I   N       M   A   T   T   E   R   %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
If we now consider an entry as in Figure \ref{fig_ch8_reco_system_linear_vs_graph_filter} - right, the linear predictor $\Phi(\bbx;\bbH)$ is expected to be uninformative but the graph filter $\Phi(\bbx;\bbh, \bbS)$ is expected to make an accurate prediction. 

\red{Link $\bbz$ to $\Phi(\bbx;\bbh, \bbS)$ and $\hbz$ to $\Phi(\hbx;\bbh, \hbS)$. If $\hbS = \bbP^T\bbS\bbP$ and $\hbx = \bbP^T\bbx$ we have that $\Phi(\hbx;\bbh, \hbS) = \bbP^T\Phi(\bbx;\bbh, \bbS)$.} 



\green{because whatever operations $\Phi(\bbx;\bbh, \bbS)$ does to predict the rating of user 3 from the ratings of users 2, 4, 8, 9, and 10 are the exact same operations that $\Phi(\bbx;\bbh, \bbS)$ would perform to predict the rating of user 6 from the ratings of users 1, 5, 7, 11, and 12. We can summarize this observation by saying that from the observations in Figure \ref{fig_ch8_reco_system_example_signals} the graph filter has learnt to predict for the input signal in the right of Figure \ref{fig_ch8_reco_system_linear_vs_graph_filter} without having ever observed this signal. This is possible because there is an inherent symmetry in graph signals that a graph filter is able to exploit. Namely, if two graph neighborhoods are similar and the signal values in the respective graph neighborhoods are similar, the outputs of a graph filter will be similar in the respective neighborhoods as well. To the extent that this invariance is an expected property in a learning task, graph filters are suitable parametrizations that will learn to process unseen examples by generalizing from examples seen in other parts of the graph with a similar structure. This is a property that holds for recommendation systems and that explains the better empirical performance of graph filter predictors relative to arbitrary linear classifiers.}

\blue{We still need to explain how these two signals are related by a permutation.}





==> ch8_sec03_gnns_old.tex <==
% !TEX root = root.tex



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t] 
\def\myfactor{1}
\centering
\input{figures/graph_perceptron.tex}
\caption{Graph Perceptron. A graph perceptron composes a graph convolutional filter with a pointwise nonlinearity. It is a minor variation of a graph filter which, among other shared properties, retains the neighborhood locality we studied in \red{Section \ref{ch_filters} of Chapter \ref{ch_filters}.}}
\label{fig_ch8_graph_perceptron}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Graph Neural Networks}\label{sec_ch8_gnns}



Graph neural networks (GNNs) extend graph filters by using pointwise nonlinearities which are nonlinear functions that are applied independently to each component of a vector. For a formal definition begin by introducing a single variable function $\sigma:\reals\to\reals$ which we extend to the vector function $\sigma:\reals^N\to\reals^N$ by independent application to each component. Thus, if we have $\bbu = [u_1; \ldots; u_N] \in \reals^N$ the output vector $\sigma(\bbu)$ is such that
% 
\begin{equation} \label{eqn_ch8_pointwise_nonlinearity}
   \sigma\big(\,\bbu\,\big) \ : \ \big[\,\sigma\big(\,\bbu\,\big)\,\big]_i = \sigma\big(\,u_i\,\big).
\end{equation}
%
I.e., the output vector is of the form $\sigma(\bbu) = [\sigma(u_1); \ldots; \sigma(u_N)]$. Observe we are abusing notation and using $\sigma$ to denote both, the scalar function and the pointwise vector function.

Recall now from our discussion in \red{Chapter \ref{ch_filters}} that graph filters are given by matrices of the form $\bbH(\bbS) := \sum_{k=0}^{\infty} h_{k} \bbS^{k}$ for a given set of coefficients $\bbh=\{h_k\}_{k=0}^\infty$. Apply this filter to a graph signal $\bbx$ to produce the graph signal
% 
\begin{equation} \label{eqn_ch8_perceptron_graph_filter}
	\bbu  \ = \ \bbH(\bbS) \bbx
	      \ = \ \sum_{k=0}^{\infty} h_{k} \bbS^{k} \bbx .
\end{equation}
%
The signal $\bbu$ is the one we use in \eqref{eqn_ch8_erm_graph_filter} as a learning parametrization. In a single layer GNN, the graph signal $\bbu$ is passed trough a pointwise nonlinear function satisfying \eqref{eqn_ch8_pointwise_nonlinearity} to produce the output.
% 
\begin{equation} \label{eqn_ch8_perceptron_nonlinearity}
	\bbz \  = \ \sigma  \Big(\, \bbu \, \Big)
	     \  = \ \sigma \Big(\,\bbH(\bbS) \bbx \, \Big)	  
	     \  = \ \sigma \Bigg (\sum_{k=0}^{\infty} h_{k} \bbS^{k} \bbx \Bigg) .
\end{equation}
%
We say the transform in \eqref{eqn_ch8_perceptron_nonlinearity} is a graph perceptron; see Figure \ref{fig_ch8_graph_perceptron}. Different from most other graph signal processing methods introduced in this book, the graph perceptron is a nonlinear function of the input. It is, however, a very simple form of nonlinear processing because the nonlinearity does not mix signal components. Signal components are mixed by the graph filter but are then processed element-wise through $\sigma$. In particular, \eqref{eqn_ch8_perceptron_nonlinearity} retains the locality properties of graph convolutional filters -- \red{see Section \ref{ch_filters} in Chapter  \ref{ch_filters}}. We will see later that other appealing properties are also shared by graph filters and GNNs.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t] 
\def\myfactor{1}
\centering
\input{figures/gnn_block_diagram_single_feature}%\\ {\small (a)}
\caption{Graph Neural Network (GNN). GNNs are compositions of layers each of which composes graph filters $\bbH_l(\bbS)=\sum_{k=0}^\infty h_{lk}\bbS^k$ with pointwise nonlinearities $\sigma$ [cf.  \eqref{eqn_ch8_gnn_recursion_single_feature_filter} and \eqref{eqn_ch8_gnn_recursion_single_feature_nonlinearity}]. The output $\Phi (\bbx; \bbH, \bbS) = \bbx_L = \bbx_3$ in this example follows at the end of a cascade of 3 layers recursively applied to the input $\bbx$. Layers are defined by sets of coefficients grouped in the tensor $\bbH:=\{\bbh_1, \bbh_2, \bbh_3\}$ which is chosen to minimize a training loss for a given shift $\bbS$ [cf. \eqref{eqn_ch8_erm_linear}].}
\label{fig_ch8_gnn_block_diagram}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\subsection{Multiple Layers}\label{sec_ch8_gnns_multiple_layers}

Graph perceptrons can be stacked in layers to create (multilayer) GNNs -- see Figure \ref{fig_ch8_gnn_block_diagram}. This stacking is mathematically written as a function composition where the outputs of a layer become inputs to the next layer. For a formal definition let $l=1,\ldots,L$ be a layer index and $\bbh_l=\{h_{lk}\}_{k=0}^\infty$ be a collection of $L$ graph filter coefficients that define a respective collection of $L$ graph filters $\bbH_l(\bbS)=\sum_{k=0}^\infty h_{lk}\bbS^k$. At layer $l$ we take as input the output $\bbx_l$ of layer $l-1$ which we process with the filter $\bbH_l(\bbS)$ to produce the intermediate feature
% 
\begin{align}\label{eqn_ch8_gnn_recursion_single_feature_filter}
   \bbu_{l} \ = \ \bbH_l(\bbS)\, \bbx_{l-1} 
            \ = \ \sum_{k=0}^\infty h_{lk}\bbS^k\, \bbx_{l-1},
\end{align} 
%
where, by convention, we say that $\bbx_0 = \bbx$ so that the given graph signal $\bbx$ is the GNN input. As in the case of the graph perceptron, this feature is passed through a pointwise nonlinear function to produce the $l$th layer output
% 
\begin{align}\label{eqn_ch8_gnn_recursion_single_feature_nonlinearity}
   \bbx_{l} \ = \ \sigma(\bbu_l )  
            \ = \ \sigma\Big(\bbH_l(\bbS)\, \bbx_{l-1} \Big)  
            \ = \ \sigma\Bigg(\sum_{k=0}^\infty h_{lk}\bbS^k\, \bbx_{l-1}\Bigg) ,
\end{align} 
%
After recursive repetition of \eqref{eqn_ch8_gnn_recursion_single_feature_filter}-\eqref{eqn_ch8_gnn_recursion_single_feature_nonlinearity} for $l=1,\ldots,L$ we reach the $L$th layer whose output $\bbx_L$ is not further processed and is declared to be the GNN output $\bbz=\bbx_L$. To represent the output of the GNN we define the filter tensor $\bbH:=\{\bbh_l\}_{l=1}^L$ grouping the $L$ sets of filter coefficients at each layer and define the operator $\Phi(\,\cdot\,;\bbH,\bbS)$ as the map
% 
\begin{align}\label{eqn_ch8_gnn_operator_single_feature}
   \Phi (\bbx; \bbH, \bbS) = \bbx_L.
\end{align} 
%
We repeat that in \eqref{eqn_ch8_gnn_operator_single_feature} the GNN output $\Phi (\bbx; \bbH, \bbS) = \bbx_L$ follows from recursive application of \eqref{eqn_ch8_gnn_recursion_single_feature_filter}-\eqref{eqn_ch8_gnn_recursion_single_feature_nonlinearity} for $l=1,\ldots,L$ with $\bbx_0=\bbx$. Observe that this operator notation remarks that the output of a GNN depends on the filter tensor $\bbH$ and the graph shift operator $\bbS$. 

A block diagram for a GNN with $L=3$ layers is shown in Figure \ref{fig_ch8_gnn_block_diagram}. The input $\bbx$ is fed to the first layer where it is processed by the filter $\bbH_1(\bbS)=\sum_{k=0}^\infty h_{1k}\bbS^k$ and passed through the pointwise nonlinearity $\sigma$ to produce the first layer output 
%
\begin{align}\label{eqn_ch8_gnn_single_feature_layer_1}
   \bbx_{1} = \sigma\Bigg(\sum_{k=0}^\infty h_{1k}\bbS^k\, \bbx \Bigg).
\end{align}
%
This is according to \eqref{eqn_ch8_gnn_recursion_single_feature_filter}-\eqref{eqn_ch8_gnn_recursion_single_feature_nonlinearity} with $l=1$ and $\bbx_0=\bbx$. The output of Layer 1 is sent to Layer 2 where it is processed by the filter $\bbH_2(\bbS)=\sum_{k=0}^\infty h_{2k}\bbS^k$ and passed through the pointwise nonlinearity $\sigma$ to produce the Layer 2 output 
%
\begin{align}\label{eqn_ch8_gnn_single_feature_layer_2}
   \bbx_{2} = \sigma\Bigg(\sum_{k=0}^\infty h_{2k}\bbS^k\, \bbx_1\Bigg),
\end{align}
%
as per \eqref{eqn_ch8_gnn_recursion_single_feature_filter}-\eqref{eqn_ch8_gnn_recursion_single_feature_nonlinearity} with $l=2$. This output becomes an input to Layer 3 where it is processed to produce the Layer 3 output 
%
\begin{align}\label{eqn_ch8_gnn_single_feature_layer_3}
   \bbx_{3} = \sigma\Bigg(\sum_{k=0}^\infty h_{3k}\bbS^k\, \bbx_2\Bigg),
\end{align}
%
again, as dictated by \eqref{eqn_ch8_gnn_recursion_single_feature_filter}-\eqref{eqn_ch8_gnn_recursion_single_feature_nonlinearity}. Since this is a GNN with $L=3$ layers, this becomes the output of the GNN $\Phi (\bbx; \bbH, \bbS) = \bbx_L = \bbx_3$. Observe that each layer is defined by a set of filter coefficients that are grouped in the tensor $\bbH:=\{\bbh_1, \bbh_2, \bbh_3\}$. These sets of coefficients are chosen to minimize a training loss for a given shift operator $\bbS$ as we explain in Section \ref{sec_ch8_gnns_training_architectures}.

\paragraph{Increasing Representation Power.} The class of functions that can be represented with all possible perceptrons is larger than the class of functions that can be represented with all possible graph filters. This is because the latter are linear functions while the former are nonlinear. The class of functions that can be represented with a multilayer GNN is, in turn, larger than the class of functions representable with a perceptron. This is true because the composition of perceptrons is not a graph perceptron. This is to be contrasted with a composition of graph filters which is also a graph filter. If, for example, $\bbH_1(\bbS)$ and $\bbH_2(\bbS)$ are graph filters, their composition is the product $\bbH_1(\bbS)\bbH_2(\bbS)$ which can be written as a polynomial on $\bbS$ and is therefore also a graph filter. Thus, a composition of graph filters would not enlarge the class of representable functions. But a composition of perceptrons does.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t] 
\def\myfactor{1}
\centering
\input{figures/gnn_block_diagram_mimo_filter}%\\ {\small (a)}
\caption{Graph Neural Network (GNN) with Multiple Features. We expand the repreesentation power of GNNs with the addition of multiple features per layer [cf. \eqref{eqn_ch8_gnn_features}]. The graph filters in each layer are multiple-input-multiple-output graph filters (cf. \eqref{eqn_ch8_gnn_recursion_filter_matrix}]. They take $F_{l-1}$ graph signals as inputs and produce $F_l$ graph signals as outputs. The structure is otherwise identical to the single feature GNN in Figure \ref{fig_ch8_gnn_block_diagram}.}
\label{fig_ch8_gnn_block_diagram_mimo}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\subsection{Multiple Features}\label{sec_ch8_gnn_multiple_features}

To further increase the representation power of GNNs we incorporate multiple features per layer that are the result of processing multiple input features with a bank of graph filters; see Figure \ref{fig_ch8_gnn_block_diagram_mimo}. For a formal definition let $F_l$ be the number of features at Layer $l$ and define the corresponding feature matrix as
% 
\begin{equation} \label{eqn_ch8_gnn_features}
   \bbX_l = \left[ \bbx_{l}^{1},\, \bbx_{l}^{2},\, \ldots,\, \bbx_{l}^{F_l} \right].
\end{equation}
%
We have that $\bbX_l\in\reals^{n\times F_l}$ and interpret each column of $\bbX_l$ as a graph signal. The outputs of Layer $l-1$ are inputs to Layer $l$ where the set of $F_{l-1}$ features in $\bbX_{l-1}$ are processed by a filterbank made up of $F_{l-1}\times F_l$ filters. For a compact representation of this bank consider coefficient matrices $\bbH_{lk}\in\reals^{F_{l-1}\times F_l}$ to build the intermediate feature matrix
% 
\begin{align}\label{eqn_ch8_gnn_recursion_filter_matrix}
   \bbU_{l} \ = \ \sum_{k=0}^\infty \bbS^k\, \bbX_{l-1}\, \bbH_{lk} \ .
\end{align} 
%
Each of the $F_l$ columns of the matrix $\bbU_l\in\reals^{n\times F_l}$ is a separate graph signal. We say that \eqref{eqn_ch8_gnn_recursion_filter_matrix} represents a multiple-input-multiple-output graph filter since it takes $F_{l-1}$ graph signals as inputs and yields $F_{l}$ graph signals at its output. As in the case of the single feature GNN of Section \ref{sec_ch8_gnns_multiple_layers} -- and the graph perceptron in \eqref{eqn_ch8_perceptron_nonlinearity} -- the intermediate feature $\bbU_{l}$ is passed through a pointwise nonlinearity to produce the $l$th layer output
% 
\begin{align}\label{eqn_ch8_gnn_recursion_nonlinearity_matrix}
   \bbX_{l} \ = \ \sigma(\bbU_l )  
            \ = \ \sigma\Bigg(\sum_{k=0}^\infty \bbS^k\, \bbX_{l-1}\, \bbH_{lk} \Bigg).
\end{align} 
%
When $l=0$ we convene that $\bbX_0=\bbX$ is the input to the GNN which is made of $F_0$ graph signals. The output $\bbX_L$ of layer $L$ is also the output of the GNN which is made up of $F_L$ graph signals. To define a GNN operator we group filter coefficients $\bbH_{lk}$ in the tensor $\bbH = \{\bbH_{lk}\}_{l,k}$ and define the GNN operator
% 
\begin{align}\label{eqn_ch8_gnn_operator_multifeature}
   \Phi (\bbX; \bbH, \bbS) = \bbX_L.
\end{align} 
%
If the input is a single graph signal as in \eqref{eqn_ch8_perceptron_nonlinearity} and \eqref{eqn_ch8_gnn_operator_single_feature}, we have $F_0=1$ and $\bbX_0=\bbx\in\reals^n$. If the output is also a single graph signal -- as is also the case in \eqref{eqn_ch8_perceptron_nonlinearity} and \eqref{eqn_ch8_gnn_operator_single_feature} -- we have $F_L=1$ and $\bbX_L=\bbx_L\in\reals^n$. 

To better understand the GNN defined by recursive application of \eqref{eqn_ch8_gnn_recursion_filter_matrix} and \eqref{eqn_ch8_gnn_recursion_nonlinearity_matrix} it is instructive to separate the matrix of filter coefficients $\bbH_{lk}$ into its individual entries. Denote then as $h_{lk}^{fg} = [\bbH_{lk}]_{fg}$ the $(f,g)$ entry of $\bbH_{lk}$ and consider application of filter coefficients  $h_{lk}^{fg}$ to the input feature $\bbx_{l-1}^f = [\bbX_{l-1}]_{f}$ stored in the $f$th column of $\bbx_{l-1}$. This results in graph signals
% 
\begin{equation} \label{eqn_ch8_gnn_filter}
	\bbv_l^{fg} \ = \ \bbH_l^{fg}(\bbS)\, \bbx_{l-1}^f  
	            \ = \ \sum_{k=0}^{\infty} h_{lk}^{fg}\, \bbS^{k} \bbx_{l-1}^f .
\end{equation}
%
Each of the $\bbv_l^{fg}\in\reals^n$ is a graph signal produced from input feature $\bbx_{l-1}^f$ through application of the filter defined by the set of coefficients $\bbh_l^{fg}=\{h_{lk}^{fg}\}_{k=0}^\infty$. Since there are $F_l$ filters associated to each fixed $f$, each of the input features $\bbx_{l-1}^f$ generates $F_l$ features $\bbv_l^{fg}$. This yields a total of $F_{l-1}\times F_l$ features which we reduce to $F_l$ features with a simple addition of all the features $\bbv_l^{fg}$ for a fixed $f$,
% 
\begin{equation} \label{eqn_ch8_gnn_filter_addition}
	\bbu_l^{g} \ = \ \sum_{f=0}^{F_{l-1}} \bbv_l^{fg}.
% 	           \ = \ \sum_{g=0}^{F_{l-1}} 
%	                        \Bigg(\sum_{k=0}^{\infty} h_{lk}^{fg}\, \bbS^{k} \bbx_{l-1}^f\Bigg)
\end{equation}
%
Each of the features $\bbu_l^{g}$ is a graph signal. There are $F_l$ of them and it is ready to see that they corresponds to the columns of $\bbU_l = [\bbu_l^1,\ldots,\bbu_l^{F_l}]$. These features can now be processed with a pointwise nonlinearity to yield the $l$th layer output feature $g$ as 
% 
\begin{equation} \label{eqn_gnn_nonlinearity}
   \bbx_{l}^{g} \ = \ \sigma \Big(\, \bbu_l^{g} \Big).
%                  \ = \ \sigma \Bigg(\, \sum_{f=1}^{F_l} \bbv_l^{fg}\, \Bigg).
\end{equation}
%
Since the nonlinearity is pointwise and we have already established that $\bbU_l = [\bbu_l^1,\ldots,\bbu_l^{F_l}]$ it follows that $\bbX_l = [\bbx_l^1,\ldots,\bbx_l^{F_l}]$. I.e., the output feature $\bbx_{l}^{g}$ is the $g$th column of the feature matrix $\bbX_l$.

The explicit expansion of \eqref{eqn_ch8_gnn_recursion_filter_matrix}-\eqref{eqn_ch8_gnn_recursion_nonlinearity_matrix} into \eqref{eqn_ch8_gnn_filter}-\eqref{eqn_gnn_nonlinearity} provides a clearer view of the processing that goes on into each layer of the GNN. Input features $\bbx_l^f$ are processed by a separate filter banks made up of the $F_l$ filters $\bbH_l^{fg}(\bbS)$ with matching index $f$. The effect of applying these parallel filterbanks is a set of $F_{l-1}\times F_l$ features $\bbv_l^{fg}$. If these were directly processed with a pointwise nonlinearity we would experience an exponential growth in the number of features as we add more layers. To avoid this exponential growth we add all of the features $\bbv_l^{fg}$ for a fixed $f$ to create the graph signal $\bbu_l^{g}$. There are $F_l$ of these which we pass through a pointwise nonlinearity to yield the $l$th layer output features $\bbx_l^{g}$ with $g=1,\ldots,F_l$. The expressions in \eqref{eqn_ch8_gnn_recursion_filter_matrix}-\eqref{eqn_ch8_gnn_recursion_nonlinearity_matrix} are just a more compact notation for the same set of operations. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t] 
\def\myfactor{1}
\centering
\input{figures/gnn_multiple_features}%\\ {\small (a)}
\caption{Graph Neural Network (GNN) with Multiple Features. Alternative representation of Figure \ref{fig_ch8_gnn_block_diagram_mimo} where the multiple-input-multiple-output graph filters at each layer are represented in expanded form.}
\label{fig_ch8_gnn_block_diagram_mimo_expanded}
\end{figure}

A GNN with 3 layers and multiple features per layer is shown in its expanded form in Figure \ref{fig_ch8_gnn_block_diagram_mimo_expanded}. Begin with layer $l=1$, whose input is a single given graph signal $\bbx$. Instead of processing $\bbx$ with a single filter, we process it through a parallel bank of $F_1=2$ filters. Processing the input signal $\bbx$ produces the collection of $F=2$ intermediate features,
% 
\begin{equation} \label{eqn_ch8_gnn_mf_layer1_filter}
	\bbv_1^{1g} \ = \ \bbH_1^{1g}(\bbS)\, \bbx 
	           \ = \ \sum_{k=0}^{\infty} h_{1k}^{1g}\, \bbS^{k} \bbx.         	   
\end{equation}
%
Each of these features is now {\it separately} passed through a pointwise nonlinearity to produce the layer 1 output features
% 
\begin{equation} \label{eqn_ch8_gnn_mf_layer1_filter_nonlinearity}
	\bbx_1^{g}  \ = \ \sigma (\bbv_1^{1g})
\end{equation}
%
There is no sum here as in \eqref{eqn_ch8_gnn_filter_addition} because $F_0=1$. I.e., because layer 1 receives a single graph signal as input. 

Different from Section \ref{sec_ch8_gnns_multiple_layers}, Layer 1 produces now a collection of $F_1$ output features. Each of these features becomes an input to Layer 2 where is now separately processed with a filterbank made up of $F_2=2$ filters. This means we have a total of $F_1 \times F_2 = 4$ filters that we index by $f=1,2$ and $g=1,2$. The filter coefficients are given by coefficient sets $\bbh_{2}^{fg} = \{h_{2k}^{fg}\}_{k=0}^\infty$. The processing of input feature $f$ with filter $\bbh_{2}^{fg}$ produces the intermediate feature
% 
\begin{equation} \label{eqn_ch8_gnn_mf_layer2_filter}
	\bbv_2^{fg} \ = \ \bbH_2^{fg}(\bbS)\, \bbx 
	            \ = \ \sum_{k=0}^{\infty} h_{2k}^{fg}\, \bbS^{k} \bbx_1^{f}.         	   
\end{equation}
%
The 4 features described by \eqref{eqn_ch8_gnn_mf_layer2_filter} are now summed up and passed through a pointwise nonlinearity to produce the two output features,
% 
\begin{equation} \label{eqn_ch8_gnn_mf_layer2_nonlinearity}
	\bbx_2^{g} \ = \ \sigma \Big[\, \bbv_2^{1g} + \bbv_2^{2g} \, \Big] ,
\end{equation}
%
for $g=1,2$. We have combined steps \eqref{eqn_ch8_gnn_filter_addition} and \eqref{eqn_gnn_nonlinearity} into \eqref{eqn_ch8_gnn_mf_layer2_nonlinearity}. We emphasize the crosstalk in the block diagram in Figure \ref{fig_ch8_gnn_block_diagram_mimo_expanded}. The two input features $\bbx_1^{1}$ and $\bbx_1^{2}$ affect the two output features $\bbx_2^{1}$ and $\bbx_2^{2}$. This is always true of GNN layers of the form in \eqref{eqn_ch8_gnn_filter}-\eqref{eqn_gnn_nonlinearity}. All the features $\bbx_{l-1}^{f}$ that are fed to layer $l$ may have an effect on all output features $\bbx_{l}^{g}$.

The 2 features generated by Layer 2 are now fed to Layer 3, which is also the output layer of this GNN. We are considering a single output GNN with $F_L=F_3=1$. Thus, we have $F_2 \times F_3 = 2$ filters in this layer. Each of these filters separately processes each of the input features to compute the graph signals
% 
\begin{equation} \label{eqn_ch8_gnn_mf_layer3_filter}
	\bbv_3^{f1} \ = \ \bbH_3^{f1}(\bbS)\, \bbx 
	            \ = \ \sum_{k=0}^{\infty} h_{3k}^{f1}\, \bbS^{k} \bbx_2^{f}.         	   
\end{equation}
%
The 2 features described by \eqref{eqn_ch8_gnn_mf_layer3_filter} are now summed up and passed through a pointwise nonlinearity to produce the single output feature,
% 
\begin{equation} \label{eqn_ch8_gnn_mf_layer3_nonlinearity}
	\bbx_3^{1} \ = \ \sigma \Big[\, \bbv_3^{11} + \bbv_3^{21} \, \Big] .
\end{equation}
%
As in \eqref{eqn_ch8_gnn_mf_layer2_nonlinearity}, we have combined steps \eqref{eqn_ch8_gnn_filter_addition} and \eqref{eqn_gnn_nonlinearity} into \eqref{eqn_ch8_gnn_mf_layer2_nonlinearity}. The signal in \eqref{eqn_ch8_gnn_mf_layer3_nonlinearity} is the output of this GNN, 
% 
\begin{equation} \label{eqn_ch8_gnn_mf_output}
	\bbPhi(\bbx; \bbH, \bbS) = \bbx_3^1.
\end{equation}
%
Output values are determined by the input signal $\bbx$, the shift operator $\bbS$, and the filter tensor $\bbH=\{ \bbh_{1}^{11}, \bbh_{1}^{12}, \bbh_{2}^{11}, \bbh_{2}^{21}, \bbh_{2}^{12}, \bbh_{2}^{22}, \bbh_{3}^{11}, \bbh_{3}^{21}\}$. This tensor is trained to minimize a loss over a distribution of graph signals for a given shift operator as we explain in the next section.

\paragraph{Arbitrary Feature Combinations.} Just adding the signals $\bbv_l^{fg}$ in \eqref{eqn_ch8_gnn_filter_addition} seems arbitrary. Having general linear combinations of features and having some output features $\bbx_{l}^g$ being dependent on only a subset of input features $\bbx_{l-1}^f$ seems more general. There is no difference, however. Since the filter coefficients in the tensor $\bbH$ are trained (Section \ref{sec_ch8_gnns_training_architectures}), it is equivalent to search for optimal filter coefficients if they are added up or if they are linearly combined. The latter is just a scaling of filter coefficients. In particular, this includes cases in which some input features $\bbx_{l-1}^f$ do not influence some output features $\bbx_{l}^g$. This could be accomplished by excluding index $f$ from the summation in \eqref{eqn_ch8_gnn_filter_addition} but this is equivalent to having a filter $\bbh_{l}^{fg}$ with all-zero coefficients.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\subsection{Training and architectures}\label{sec_ch8_gnns_training_architectures}

As is the case of graph filters, the  output of the GNN depends on the filter tensor $\bbH$ and the shift operator $\bbS$. But when performing training we assume $\bbS$ is given and search over all possible filter tensors. To make this unambiguous, consider an extension of the training set in \eqref{eqn_ch8_training_set} in which we are given pairs of multi-feature graph signals 
% 
\begin{align}\label{eqn_ch8_training_set_mf}
   \ccalT:= \big\{(\bbX_s, \bbY_s) \big\}_{s=1}^{S},
\end{align}   
%
where $\bbX_s\in\reals^{F_0}$ and $\bbY_s\in\reals^{F_L}$. We want to train the GNN operator in \eqref{eqn_ch8_gnn_operator_multifeature} by finding a tensor $\bbH^*$ that yields the best possible output estimates
% 
\begin{align}\label{eqn_ch8_gnn_estimates_mf}
   \hbY = \bbPhi (\bbX; \bbH^*, \bbS)
\end{align}   
%
for input features $\bbX$. Given the training set in \eqref{eqn_ch8_training_set_mf} and a loss function $\ell(\hbY, \bbY)$ the optimal filter tensor is defined as the one that minimizes the empirical loss
% 
\begin{align}\label{eqn_ch8_erm_gnn_mf}
   \bbH^* \  = \ \argmin_{\bbH} \frac{1}{S} \sum_{s=1}^{S} 
                   \ell \big( \bbPhi (\bbX_s; \bbH, \bbS) , \bbY_s \big) .
\end{align} 
%
In most forthcoming examples in this chapter we work with learning tasks involving inputs and outputs made up of single graph signals. In such cases the training set in \eqref{eqn_ch8_training_set_mf} is the same as the training set in \eqref{eqn_ch8_training_set} and the matrices $\bbX$, $\bbY$, and $\hbY$ in \eqref{eqn_ch8_training_set_mf} and \eqref{eqn_ch8_erm_gnn_mf} become vectors. Just to avoid confusion in future referencing we write GNN estimates as
% 
\begin{align}\label{eqn_ch8_gnn_estimates}
   \hby = \bbPhi (\bbx; \bbH^*, \bbS)
\end{align}   
%
and define the optimal tensor as
% 
\begin{align}\label{eqn_ch8_erm_gnn}
   \bbH^* \  = \ \argmin_{\bbH} \frac{1}{S} \sum_{s=1}^{S} 
                   \ell \big( \bbPhi (\bbx_s; \bbH, \bbS) , \bby_s \big) .
\end{align} 
%
Notice that even if $\bbx$ and $\bby$ are single feature vectors it is still desirable to have intermediate layers with multiple features as in Figure \ref{fig_ch8_gnn_block_diagram_mimo_expanded}.

When training \eqref{eqn_ch8_erm_gnn_mf} or \eqref{eqn_ch8_erm_gnn} the search is over tensors whose form depends on: (i) The number of layers $L$. (ii) The number of features per layer $F_0, \ldots, F_L$. In practice, the number of filter taps, which is assumed infinite in \eqref{eqn_ch8_gnn_recursion_filter_matrix} is also limited. This adds a third limitation to the class of allowable filters: (iii) The number of filter taps $K_1, \ldots, K_L$ allowed at each layer.  The collection of these three types of parameters defines what we call a GNN architecture,
% 
\begin{align}\label{eqn_ch8_gnn_architecture}
   \ccalH = \{ L, F_0, (F_1, K_1), \ldots, (F_L, K_L) \}.
\end{align} 
%
The specification of the parameters in \eqref{eqn_ch8_gnn_architecture} determines the type of GNN restricts the tensor search in \eqref{eqn_ch8_erm_gnn_mf} or \eqref{eqn_ch8_erm_gnn}. Suppose that in Figure \ref{fig_ch8_gnn_block_diagram_mimo_expanded} we choose to use filters of length $K_l=5$ for all layers. In such case we would have $\ccalH=\{3, 1, (2,5), (2,5), (1,5)\}$.



==> ch8_sec03_stability_of_graph_filters.tex <==
% !TEX root = ../compile_all_book/gsp.tex



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Effect of Absolute Graph Perturbations on Graph Filters}\label{sec_graph_perturbations}

To understand the stability of graph filters it is instructive to consider the form of \eqref{eqn:graphFilter} in the graph frequency domain. This entails using the eigenvector basis $\bbV$ in \eqref{eqn:eigendecomposition} to define the {\it Graph Fourier Transform} (GFT) of the graph signal $\bbx$ as the projection $\tbx = \bbV^{\Hr}\bbx$ \cite{Sandryhaila14-Freq}. Substituting the GFT definition in the definition of the graph convolution in \eqref{eqn:graphFilter} and using the fact that $\bbS^k = \bbV\bbLam^k\bbV^{\Hr}$ we can write 
% 
\begin{equation} \label{eqn:filter_dft}
   \bbV^{\Hr}\bbz \ =\  \tbz \ 
	          \ = \ \sum_{k=0}^{\infty} h_{k}\bbLam^{k}\big(\bbV^{\Hr}\bbx\big)
	          \ = \ \bbH(\bbLam) \hbx .
\end{equation}
%
The interesting conclusion that follows from \eqref{eqn:filter_dft} is that graph filters are pointwise operators in the graph frequency domain because $\bbH(\bbLam)$ is a diagonal matrix. This motivates the definition of the graph frequency response as the analytic function $h:\reals\to\reals$ defined by the graph filter coefficients $\bbh = \{h_{k}\}_{k=0}^\infty$,  
% 
\begin{equation} \label{eqn:frequency_response}
	h(\lam)  \ = \ \sum_{k=0}^{\infty} h_{k} \lam^{k} .
\end{equation}
%
Comparing \eqref{eqn:filter_dft} with \eqref{eqn:frequency_response} we conclude that the $i$th component $\tdx_i$ of the input signal GFT $\tbx$ and  the $i$th component $\tdz_i$ of the output signal GFT $\tbz$ are related through the expression
% 
\begin{equation} \label{eqn:frequency_response_pointwise}
	\tdz_i = h(\lam_i) \tdx_i.
\end{equation}
%
The remarkable observation to be made at this point is that the frequency response of a filter is completely characterized by the filter coefficients $\bbh$ [cf. \eqref{eqn:frequency_response}]. The effect of a specific graph is to determine the components of the GFT $\tbx = \bbV^{\Hr}\bbx$ -- through its eigenvectors $\bbV$ -- and which values of the frequency response are instantiated [cf. \eqref{eqn:frequency_response_pointwise}] -- through its eigenvalues $\bbLam$. Figure \ref{fig_frequency_response} shows an illustration of this latter fact. We have a filter with frequency response $h(\lam)$ represented as a continuous function. For a graph with eigenvalues $\lam_i$ only the values at frequencies $h(\lam_i)$ affect the response of the filter. For a different graph with eigenvalues $\hlam_i$ the values $h(\hlam_i)$ are the ones that determine the effect of the filter in the given graph. 

Since graph perturbations alter the spectrum of a graph it seems apparent that the variability of the frequency response $h(\lam)$ has a direct effect on a filter's stability to perturbations. To proceed with a formal characterization we introduce the notion of Lipschitz filters in the following definition.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t]
    \centering
    \input{../ch8_gnn/figures_stability/frequency_response_instantiation.tex}    
    \caption{Frequency response of a graph filter. The function $h(\lambda)$ is shown as a black, solid line, and is independent of the graph. When evaluated on a given graph shift operator, specific values of $h$ are instantiated on the eigenvalues of the given GSO. For example, when given a GSO $\bbS$ with eigenvalues $\{\lambda_{i}\}$, the graph filter frequency response will be instantiated on $h(\lambda_{i})$ (in blue); but, if we are given a different GSO $\hbS$ with other eigenvalues $\{\hlam_{i}\}$, then the filter frequency response will be given by $h(\hlam_{i})$ (in red).}
    \label{fig_frequency_response}
\end{figure}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   D   E   F   I   N   I   T   I   O   N   %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{definition}[Lipschitz Filter]\label{def:lipschitzFilters}
Given a filter with coefficients $\bbh = \{h_{k}\}_{k=0}^\infty$ we say the filter is Lipschitz if there exists a constant $C>0$ such that for all $\lam_1$ and $\lam_2$ the frequency response $h(\lam)$ in \eqref{eqn:frequency_response} is such that
% 
\begin{equation}\label{eqn:lipschitzFilters}
   \big| h(\lam_2) - h(\lam_1) \big| 
       \leq C \big| \lam_2 - \lam_1 \big|.
\end{equation} \end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
As its name suggests, a filter is Lipschitz if its frequency response is Lipschitz. This requirement implies that a Lipschitz filter is one whose frequency response does not change faster than linear. For filters that are Lipschitz, we can prove the following stability result relative to perturbations that are close to permutations.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   T   H   E   O   R   E   M   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{theorem} \label{thm:filterStabilityAbsolute}
Let $\bbS = \bbV \bbLambda \bbV^{\Hr}$ and $\hbS$ be graph shift operators. Let $\bbE = \bbU \bbM \bbU^{\Hr}$ be the perturbation modulo permutation between $\bbS$ and $\hbS$ (cf. Definition \ref{def_operator_distance}) and assume that their relative operator distance modulo permutation (cf. Definition \ref{def_operator_distance}) satisfies
% 
\begin{equation} \label{eqn:hypothesisEabsolute}
   \| \bbS - \hbS \|_\ccalP  = \| \bbE\| \leq \eps.
\end{equation}
%
For a Lipschitz filter (cf. Definition \ref{def:lipschitzFilters}) with Lipschitz constant $C$ the operator distance modulo permutation between filters $\bbH(\bbS)$ and $\bbH(\hbS)$ satisfies
% 
\begin{equation} \label{eqn:boundFilterAbsolute}
    \| \bbH(\bbS) - \bbH(\hbS) \|_\ccalP 
        \ \leq \ C
            \left(1 + \delta\sqrt{N} \right)\eps
            + \ccalO(\eps^{2}) ,
\end{equation}
%
with $\delta := (\| \bbU - \bbV \|_{2}+1)^{2} -1$ standing for the eigenvector misalignment between  shift operator $\bbS$ and error matrix $\bbE$.
\end{theorem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   P   R   O   O   F   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{proof} See appendix \ref{sec_apx_B} \end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
To a first order approximation, Theorem \ref{thm:filterStabilityAbsolute} shows that filters are Lipschitz stable with respect to perturbations of the graph with stability constant $C (1 + \delta\sqrt{N})$ and that this is true uniformly for all graphs with a given number of nodes $N$. 

The stability constant in \eqref{eqn:boundFilterAbsolute} consists of the product of two terms. One given by the filter's Lipchitz constant $C$ and one containing the eigenvector misalignment constant $(1+\delta\sqrt{N})$. It is interesting that each of these terms represents a different facet of the graph filtering problem. The Lipschitz constant $C$ is a property of the filter which is up for choice during filter design. The term $(1+\delta\sqrt{N})$ is a property of the family of perturbations $\bbE$ that are admissible which is an inherent property of the type of perturbations we expect to see in a specific problem. It is important to remark that we can affect $C$ by designing the filter properly but we can't affect $\delta$. The latter is not a property of the filter, but a property of the perturbation $\bbE$. The important point is that, regardless of $\delta$, judicious choice of filter coefficients $\bbh$, affects the Lipschitz constant $C$ and allows control of the stability of the graph filters that we use to construct permutation equivariant features.

As per Theorem \ref{thm:filterStabilityAbsolute}, the filter stability constant with respect to perturbations of the graph is $C (1 + \delta\sqrt{N})$. Since the larger $C$ is, the more sensitive the filter is to perturbations, achieving stability to perturbations calls for restricting $C$. The cost of restricting $C$ is to limit the rate of change of the filter's response, which limits the ability to discriminate features with close spectral signatures. This is a fundamental limitation. It is impossible to have filters that are are both, highly discriminative and highly stable. That said, this is a limitation that partly stems from a perturbation model that is not fully adequate. An additive perturbation of the form in \eqref{eqn:hypothesisEabsolute} incorporates edges of order $\eps$ without regards for the magnitude of the edges $s_{ij}$. In principle, we could overcome this limitation by replacing the hypothesis in \eqref{eqn:hypothesisEabsolute} to make the error proportional to the norm of the shift operator. If we make $\| \bbS - \hbS \|_\ccalP  \leq \eps \|\bbS\|$ it follows readily that \eqref{eqn:boundFilterAbsolute} becomes 
%
\begin{equation} \label{eqn:boundFilterAbsolute_dependent_on_S}
    \| \bbH(\bbS) - \bbH(\hbS) \|_\ccalP 
        \ \leq \ C
            \left(1 + \delta\sqrt{N} \right) \|\bbS\| \eps 
            + \ccalO(\eps^{2}) .
\end{equation}
%
The bound in \eqref{eqn:boundFilterAbsolute_dependent_on_S} is the result of a {\it relative} perturbation model and shows stability with a minor modification in the stability constant which becomes $C\left(1 + \delta\sqrt{N} \right) \|\bbS\|$. The bound in \eqref{eqn:boundFilterAbsolute_dependent_on_S} still shows an unsolvable tradeoff between stability and discriminability. But it is also a model that is still not fully adequate because it ties a global property of the graph, the norm $\|\bbS\|$ of the shift operator, to a global property of the error, its norm $\|E\| \leq \eps \|\bbS\| $. In particular, this may imply that parts of the graph with small weights have large relative modifications because some other parts of the graph have large weights. 

To find bounds that mitigate this inadequacy, we pursue alternative models of relative perturbations in the following section. In the process, we will show that it is possible to have filters that are both, stable and discriminative. A fact that will motivate the introduction of graph neural networks in Section \ref{sec:graphNeuralNetworks}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\subsection{Effect of Relative Graph Perturbations on Graph Filters}\label{sec_graph_perturbations_relative}

A relative perturbation model of a symmetric matrix $\bbA$ is one in which we consider symmetric error matrices $\bbE$ to define symmetric perturbed matrices of the form
%
\begin{align} \label{eqn_relative_perturbation_no_permutation}
   \hbA = \bbA + \big(\bbE \bbA + \bbA \bbE\big) .
\end{align}
%
If matrices $\bbA$ and $\hbA$ are given, we can find a matrix $\bbE$ satisfying \eqref{eqn_relative_perturbation_no_permutation} to define a relative dissimilarity between $\bbA$ and $\hbA$. We do this in the following definition to measure relative perturbations between shift operators. As we did in Definition \ref{def_operator_distance} we also incorporate permutation invariances to account for arbitrary relabelings.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   D   E   F   I   N   I  T   I   O   N   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{definition}[Relative Perturbation Modulo Permutation] \label{def_relative_perturbation} 
Given shift operators $\bbS$ and $\hbS$ we define the set of relative perturbation matrices modulo permutation as 
%
\begin{alignat}{2} \label{eqn_def_relative_perturbation}
   \ccalE(\bbS, \hbS) 
      = \Big\{ \bbE : 
               \bbP^{\Tr}\hbS \bbP =  \bbS  + \big(\bbE \bbS + \bbS \bbE\big), 
               \bbP \in \ccalP \Big\}. \end{alignat}
\end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
In \eqref{eqn_def_relative_perturbation} we consider all the matrices $\bbE$ that allow us to write different permutations of $\hbS$ through relative perturbations of $\bbS$ of the form in \eqref{eqn_relative_perturbation_no_permutation}. The norm $\|\bbE\|$ of a given error matrix $\bbE$ associated to a given permutation $\bbP$ is a measure of relative dissimilarity between $\bbP^{\Tr}\hbS \bbP$ and $\bbS$. To measure dissimilarity between $\bbS$ and $\hbS$  modulo permutation we evaluate the error norm at the permutation that affords the smallest error norm
%
\begin{alignat}{2} \label{eqn_def_relative_perturbation}
   d(\bbS, \hbS) 
      = & \min_{\bbP \in \ccalP} \ &&  \| \bbE \|,   \nonumber \\
        & \st  && \bbP^{\Tr}\hbS \bbP =  \bbS  + \big(\bbE \bbS + \bbS \bbE\big) .
\end{alignat}
%
The dissimilarity $d(\bbS, \hbS)$ measures how different $\bbS$ and $\hbS$ are from being permutations of each as measured by a multiplicative factor $\bbE$. This multiplicative model ties weight changes to the local structure of the graph -- something that is not necessarily true of the absolute perturbation model considered in Section \ref{sec_graph_perturbations}. Specifically, if we write the entries of the perturbation matrix $\bbE \bbS + \bbS \bbE$ we see that the difference between the $(i,j)$ edges of $\bbS$ and $\bbP_0^{\Tr}\hbS \bbP_0$ is proportional to the sum of the degrees of nodes $i$ and $j$. Thus, individual graph edges are being perturbed by amounts that are proportional to the degrees of their boundary nodes. 

To study the effect of relative perturbations we can rely on the consideration of Lipschitz filters (cf. Definition \ref{def:lipschitzFilters}) but more illuminating results are possible with the introduction of integral Lipschitz filters which we define next.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   D   E   F   I   N   I   T   I   O   N   %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{definition}[Integral Lipschitz Filter]\label{def:integralLipschitzFilters}
Given a filter with coefficients $\bbh = \{h_{k}\}_{k=0}^\infty$ we say the filter is integral Lipschitz if there exists a constant $C>0$ such that for all $\lam_1$ and $\lam_2$ the frequency response $h(\lam)$ in \eqref{eqn:frequency_response} is such that
%
\begin{equation}\label{eqn:integralLipschitzFilters}
  \| h(\lam_2) - h(\lam_1) |
       \ \leq\  C\ \frac{| \lam_2 - \lam_1 |}{  |\lam_1 +  \lam_2| \,/\, 2  }\, .
\end{equation} \end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Filters satisfying \eqref{eqn:integralLipschitzFilters} are said integral Lipschitz because, as is ready to verify, their integration from 0 is a Lipschitz function. Intuitively, the condition in \eqref{eqn:integralLipschitzFilters} can be read as requiring the filter's frequency response to be Lipschitz in any interval $(\lam_1,\lam_2)$ with a Lipschitz constant that is proportional to the interval's midpoint $(|\lam_1 + \lam_2|)/2$. To see this better it is instructive to see that \eqref{eqn:integralLipschitzFilters} restricts the derivative of the impulse response to satisfy
%
\begin{equation}\label{eqn_integral_Lipschitz_derivative}
  \big|\lambda h'(\lam) \big| \leq C .
\end{equation}
%
Thus, filters that are integral Lipschitz must have frequency response that have to be flat for large $\lam$ but can vary very rapidly around $\lam=0$. This is, not coincidentally, a condition reminiscent of the scale invariance of wavelet transforms \red{\cite[\blue{Something on wavelets. If it's a book, make sure it's a chapter.}]{??}.}

For relative perturbation models and integral Lipschitz filters the following stability result holds.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   T   H   E   O   R   E   M   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{theorem} \label{thm:filterStabilityRelative}
Let $\bbS = \bbV \bbLambda \bbV^{\Hr}$ and $\hbS$ be graph shift operators. Let $\bbE = \bbU \bbM \bbU^{\Hr} \in \ccalE(\bbS,\hbS)$ be a relative perturbation matrix (cf. Definition \ref{def_relative_perturbation}) whose norm is such that 
% 
\begin{equation} \label{eqn:hypothesisEabsolute}
   d(\bbS, \hbS) \leq \| \bbE \| \leq \eps.
\end{equation}
%
For an integral Lipschitz filter (cf. Definition \ref{def:integralLipschitzFilters}) with integral Lipschitz constant $C$ the operator distance modulo permutation between filters $\bbH(\bbS)$ and $\bbH(\hbS)$ satisfies
% 
\begin{equation} \label{eqn:boundFilterRelative}
   \| \bbH(\bbS) - \bbH(\hbS) \|_\ccalP  
       \ \leq \  C \left(1 + \delta\sqrt{N} \right)\eps + \ccalO(\eps^{2}) ,
\end{equation}
%
with $\delta := (\| \bbU - \bbV \|_{2}+1)^{2} -1$ standing for the eigenvector misalignment between  shift operator $\bbS$ and error matrix $\bbE$
\end{theorem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   P   R   O   O   F   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{proof} See appendix \ref{sec_apx_C} \end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Theorem \ref{thm:filterStabilityRelative} establishes stability with respect to relative perturbations of the form introduced in Definition \ref{def_relative_perturbation}. If a matrix $\bbE$ exists that makes $\bbS$ and $\hbS$ close to permutations of each other in terms of this relative perturbations, the filters are stable with respect to the norm of the perturbation with stability constant $C \left(1 + \delta\sqrt{N} \right)$. Since the stability constant is the same constant of Theorem \ref{thm:filterStabilityAbsolute}, the same comments apply: (i) The bound holds uniformly for all graphs with $N$ nodes. (ii) Stability is affected by a term, the Lipschitz constant $C$, that is controllable through filter design (iii) Stability is further affected by a term, the eigenvector misalignment $(1+\delta\sqrt{N})$, that depends on the structure of the perturbations that are expected in a particular problem but that can't be affected by judicious filter choice. The important difference between Theorems \ref{thm:filterStabilityAbsolute} and \ref{thm:filterStabilityRelative} is that the class of filters that are admissible for stability with respect to relative perturbations is that of integral Lipschitz filters -- whereas Lipschitz filters are required for stability with respect to absolute perturbations. 

Before elaborating on the implications of allowing for integral Lipschitz filters we consider a variation of Theorem \ref{thm:filterStabilityRelative} in which we impose a structural constraint on the perturbation matrix $\bbE$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   T   H   E   O   R   E   M   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{theorem} \label{thm_filter_stability_structural_constraint} 
With the same hypotheses and definitions of Theorem \ref{thm:filterStabilityRelative} assume that there exists a matrix $\bbE \in \ccalE(\bbS,\hbS)$ that satisfies \eqref{eqn:hypothesisEabsolute} and, furthermore, is such that
% eqn:structuralConstraint
\begin{equation} \label{eqn:structuralConstraint}
   \min\left [ \left\| \frac{\bbE}{\|\bbE\|} - \bbI \right\| \, , \
               \left\| \frac{\bbE}{\|\bbE\|} + \bbI \right\|  \right] 
       \leq \varepsilon .
\end{equation}
%
Then, the operator distance modulo permutation between filters $\bbH(\bbS)$ and $\bbH(\hbS)$ satisfies
% 
\begin{equation}\label{eqn_thm_filter_stability_structural_constraint} 
   \| \bbH(\bbS) - \bbH(\hbS) \|_{\ccalP} 
        \leq  C \varepsilon + \ccalO(\varepsilon^{2}) .
\end{equation} \end{theorem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   P   R   O   O   F   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{proof} See appendix \ref{sec_apx_C} \end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The structural constraint in \eqref{eqn:structuralConstraint} requires the error matrix $\bbE$ to be a scaled identity to within a first order approximation. With this restriction on the set of admissible perturbations we can bound the eigenvector misalignment between $\bbS$ and $\bbE$ and remove the dependency that the bounds in Theorems \ref{thm:filterStabilityAbsolute} and \ref{thm:filterStabilityRelative} have on the number of nodes in the graph. The bound in \eqref{eqn_thm_filter_stability_structural_constraint} holds uniformly for all graphs independently of their number of nodes.

The integral Lipschitz filters in Theorems \ref{thm:filterStabilityRelative} and \ref{thm_filter_stability_structural_constraint} are of interest because they can be made finely discriminative at low frequencies without affecting stability. Indeed, to control stability in \eqref{eqn:boundFilterRelative} we need to limit the value of the integral Lipschitz constant $C$. This requires filter that change more slowly. In particular, for large $\lam$ the filters must be constant and can't discriminate nearby spectral features. But at values of $\lam$ close to $\lam=0$ the filters can change rapidly and can therefore be designed to discriminate (arbitrarily) close spectral features. To the extent that relative perturbations are admissible -- which, as we already pointed out, are arguably more sensible than absolute perturbations -- Theorem \ref{thm:filterStabilityRelative} shows two fundamental properties of linear graph filters: (i) They {\it cannot} be stable and discriminative of spectral features associated with large $\lam$. (ii) They {\it can} be stable and discriminative of spectral features associated with large $\lam\approx0$.

Thus, if we are interested in discriminating features associated with $\lam\approx0$, linear graph filters are sufficient. However, if we are interested in discriminating features associated with large $\lam$, linear graph filters will fail because of their sensitivity to graph perturbations. We will see in the following section that this an issue we can resolve with the introduction of pointwise nonlinearities to produce graph neural networks.

\begin{remark} \normalfont
Theorem \ref{thm_filter_stability_structural_constraint} provides a bound that is independent of graph properties. An interesting consequence of this fact is that it makes it ready to take limits as we grow the number of nodes in the graph. There is, in fact, no limit to be taken as the bound holds for all graphs. Of particular importance is the limit of a line graph in which case we partially recover the seminal stability results for scattering transforms using regular convolutions in \cite{Mallat12-Scattering}. The difference between Theorem \ref{thm_filter_stability_structural_constraint} and the results in \cite{Mallat12-Scattering} is our restriction that the perturbation matrix be close to an identity. This means we can perturb the line graph by dilating all edges or by contracting all edges. Dilations and contractions can be different for different nodes but we cannot have a mix of dilation and contraction in different parts of the line. This is allowed in \cite{Mallat12-Scattering} where perturbations are arbitrary diffeomorphisms. The reason for the relative weakness of the result is that \cite{Mallat12-Scattering} leverages extrinsic geometric information that is not available in an analysis that applies to arbitrary graphs.
\end{remark}



==> ch8_sec04_stability_of_gnns.tex <==
%!TEX root = stability.tex

\section{Graph Neural Networks} \label{sec:graphNeuralNetworks}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% SECTION : Graph Neural Networks  %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The superior performance of graph neural networks (GNNs) can be explained by the use of filter banks and nonlinearities to successfully process high frequencies in a stable manner. An arbitrary GNN with $L$ layers can be defined as follows \cite{Gama18-Architectures}. Let $\bbx_{\ell}^{f}$ be a graph signal describing the $f$-th output feature of layer $\ell$, for $f=1,\ldots,F_{\ell}$. Let $\bbH_{\ell}^{fg}$ be the linear filter that produces the part of the $f$th feature corresponding to the $g$th input feature $\bbx_{\ell-1}^{g}$, with $g = 1,\ldots,F_{\ell-1}$. Let $\sigma_{\ell}$ be the pointwise nonlinearity applied at layer $\ell$. Then, the GNN can be written as
% eqn:GNN
\begin{equation} \label{eqn:GNN}
    \bbx^{f}_{\ell}(\bbS) = \sigma_{\ell} 
        \left( 
            \sum_{g=1}^{F_{\ell-1}}
                \bbH^{fg}_{\ell}(\bbS) \bbx^{g}_{\ell-1}(\bbS)
        \right)
    \ , \
    f = 1,\ldots,F_{\ell}
\end{equation}
%
for $\ell=1,\ldots,L$. We set $\bbx_{0}^{g}(\bbS) = \bbx^{g}$ to be the input data described by $F_{0}$ features. The desired representation is collected as the output of the $L$th layer $\hby^{f}(\bbS) = \bbx_{L}^{f}(\bbS)$, and is denoted by $\hby(\bbS) = \{\hby^{f}(\bbS)\}_{f=1}^{F_{L}}$. The energy of this representation is defined as $\|\hby(\bbS)\|_{2}^{2} = \sum_{f=1}^{F} \| \hby^{f}(\bbS)\|_{2}^{2}$.

GNNs retain the two fundamental properties of integral Lipschitz filters. Namely, that they are equivariant, and that they are stable. First, we show equivariance.

%%%%%%%%%%%%%%
% PROPOSITION: prop:GNNPermutationEquivariance
%%%%%%%%%%%%%%
%
\begin{proposition}[GNN permutation equivariance] \label{prop:GNNPermutationEquivariance}
Let $\ccalG = (\ccalV, \ccalE, \ccalW)$ be a graph with GSO $\bbS$. Let $\hat{\ccalG}$ be the \emph{permuted} graph with GSO $\hbS= \bbP^{\Tr} \bbS \bbP$ for $\bbP \in \ccalP$. Denote by $\hby(\bbS, \bbx)$ the $F_{L}$-feature output of a GNN with $L$ layers applied to graph signal $\bbx$ [cf. \eqref{eqn:GNN}]. Assume that filters $\bbH_{\ell}^{fg}(\bbS)$ are obtained by the application of an analytic function $h_{\ell}^{fg} (\lambda) = \sum_{k=0}^{\infty} h_{\ell k}^{fg} \lambda^{k}$ to the GSO $\bbS$.

Then, for any graph signal $\bbx \in \reals^{N}$ it holds that
% eqn
\begin{equation}
\hby(\hbS, \bbP^{\Tr}\bbx) = \bbP^{\Tr} \hby(\bbS, \bbx).
\end{equation}
%
\end{proposition}
%
%%%%%%%%%
%% Proof:
%%%%
%
\begin{proof}
See appendix.
\end{proof}
%
%% End of Proof
%%%%%%%%%%%%%%%%

The stability result pertaining to this representation is given next.

%%%%%%%%%%
% THEOREM: thm:GNNStability
%%%%%%%%%%
%
\begin{theorem}[GNN Stability] \label{thm:GNNStability}
Let $\ccalG = (\ccalV, \ccalE, \ccalW)$ be a graph with GSO $\bbS = \bbV \bbLambda \bbV^{\Hr}$ and $\hat{\ccalG}$ be another graph with GSO $\hbS$ such that [cf. \eqref{eqn:graphDistanceRelative}]
% eqn:hypothesisDistanceGNN
\begin{equation} \label{eqn:hypothesisDistanceGNN}
    d(\hbS, \bbS ) \leq \varepsilon / 2.
\end{equation}
%
Let $\bbE \in \ccalE_{R}(\bbS,\hbS)$ [cf. \eqref{eqn:relativePerturbation}] such that $\bbE = \argmin d(\bbS, \hbS)$. Further consider $\bbE$ to be a normal matrix with eigendecomposition $\bbE = \bbU \bbM \bbU^{\Hr}$, with eigenvalues $m_{n}$ ordered such that $|m_{1}| \leq \cdots \leq |m_{N}|$. Relative error matrix $\bbE$ also satisfies the structural constraint [cf. \eqref{eqn:hypothesisErelative}]
% eqn:hypothesisEGNN
\begin{equation} \label{eqn:hypothesisEGNN}
    \left\| \frac{\bbE}{m_{N}} - \bbI \right\|_{2} \leq \varepsilon.
\end{equation}
%
Let $\hby(\bbS)$ be the $F_{L}$-feature output of a GNN with $L$ layers [cf. \eqref{eqn:GNN}]. Assume that filters $\bbH_{\ell}^{fg}(\bbS)$ are obtained by the application of an analytic function $h_{\ell}^{fg} (\lambda) = \sum_{k=0}^{\infty} h_{\ell k}^{fg} \lambda^{k}$ to the GSO $\bbS$ and that these filters conform a frame
% eqn:filterFrameGNN
\begin{equation} \label{eqn:filterFrameGNN}
    A^{2} \|\bbx\|_{2}^{2} 
        \leq \sum_{g=1}^{F_{\ell-1}} \|\bbH_{\ell}^{fg}(\bbS)\bbx\|_{2}^{2} 
        \leq B^{2} \| \bbx\|_{2}^{2}
\end{equation}
%
for some $0 < A \leq B < \infty$, for all $f=1,\ldots,F_{\ell}$, for all $\ell=1,\ldots,L$. They also satisfy $|\lambda (h_{\ell}^{fg}(\lambda))'| \leq C$ [cf. \eqref{eqn:integralLipschitzFilters}]. We further assume that all the pointwise nonlinearities $\sigma_{\ell}:\reals \to \reals$ are Lipschitz continuous $| \sigma_{\ell}(x) - \sigma_{\ell}(\hhatx) | \leq C_{\sigma} | x - \hhatx |$ [cf. \eqref{eqn:lipschitzFilters}] so that
% eqn:lipschitzNonlinearityGNN
\begin{equation} \label{eqn:lipschitzNonlinearityGNN}
    \| \sigma_{\ell}(\bbx) - \sigma_{\ell}(\hbx) \|_{2} 
        \leq C_{\sigma} \| \bbx - \hbx \|_{2}.
\end{equation}
%

Then, it holds that
% eqn:stabilityBoundGNN
\begin{equation} \label{eqn:stabilityBoundGNN}
    \| \hby(\bbS) - \hby(\hbS) \|_{2} 
        \leq 
            \varepsilon
            B^{L-1}
            C
            \sum_{\ell=1}^{L} 
                C_{\sigma}^{\ell} 
                \sqrt{F_{L}}\prod_{\ell=1}^{L-1}F_{\ell} 
            \sum_{g=1}^{F_{0}} \| \bbx^{g} \|_{2}.
\end{equation}
%
\end{theorem}
%
%%%%%%%%%
%% Proof:
%%%%
%
\begin{proof}
See appendix.
\end{proof}
%
%% End of Proof
%%%%%%%%%%%%%%%%

Theorem~\ref{thm:GNNStability} establishes how the stability is affected by the hyperparameters of the architecture. Most importantly, we see that the result is linear in the size $\varepsilon$ of the perturbation. We note that the deeper the GNN the larger the bound gets. Also, that the amplification factor $B$ increases the bound exponentially on the number of layers. We observe that choosing values of $B < 1$, while decreasing the gap, it actually decreases the energy of the signal from each layer to the next and, as such, it might also lose relevant information. This suggests that we should train the graph filter coefficients to have a $B \approx 1$. The  number of features also increases the gap in multiplicative fashion (due to the number of filters). With respect to the nonlinearity, we observe that many of the typically chosen nonlinearities such as ReLUs or absolute values have Lipschitz constant $C_{\sigma}=1$. While bound \eqref{eqn:stabilityBoundGNN} is not tight, we observe that, in general, the more descriptive an architecture, the larger the gap is. This is intuitively satisfying since the more elements that are there in the architecture, the more compounded the perturbation error gets. Finally, to aid in the clarity of Theorem~\ref{thm:GNNStability} we present the form the result adopts when applied to a single-layer GNN with a single input feature.

%%%%%%%%%%%%
% COROLLARY: cor:singleLayerStability
%%%%%%%%%%%%
%
\begin{corollary} \label{cor:singleLayerStability}
Under the conditions of Theorem~\ref{thm:GNNStability}, let $L=1$ in \eqref{eqn:GNN} and let the number of input features be $F_{0} = 1$ and  the number of output features be $F_{1}=F$. Then, it holds that
% eqn
\begin{equation}
    \| \hby(\bbS) - \hby(\hbS) \|_{2} 
        \leq \varepsilon C_{\sigma} C \sqrt{F} \| \bbx \|_{2}.
\end{equation}
%
\end{corollary}
%
%%%%%%%%%
%% Proof:
%%%%
%
\begin{proof}
See appendix.
\end{proof}
%
%% End of Proof
%%%%%%%%%%%%%%%%

\noindent From Corollary~\ref{cor:singleLayerStability} we see that the stability gap depends linearly on the perturbation $\varepsilon$, on the Lipschitz constant of the nonlinearity $C_{\sigma}$ and on the integral Lipschitz constant of the filters $C$. It also depends linearly on the energy of the input signal $\bbx$ and as a square root of the number of output features. We observe it does not depend on the amplification factor $B$.

==> ch8_sec05_discussions.tex <==
% !TEX root = ../compile_all_book/gsp.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Discussions}\label{sec_linear_filters_stability}

To illustrate the importance of Theorem \ref{thm:filterStabilityRelative} we discuss an illustrative example. Suppose that we have shift operators $\bbS$ and $\hbS$ where the latter is a simple scaling of the former by a factor $(1-\alpha)$
%
\begin{equation}\label{eqn:graphDilation}
   \hbS = (1-\alpha)\bbS .
\end{equation}
%
The graph dilation in \eqref{eqn:graphDilation} produces a graph in which all edges are scaled by a $(1-\alpha)$ factor. This is a perturbation model of the form in \eqref{eqn:relativePerturbation} with $\bbE=(-\alpha/2)\bbI$. We consider that $\alpha\approx0$ in which case the graph dilation produces a minimal modification of the graph.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t]
    \centering
    \input{../ch8_gnn/figures_stability/graph_dilation_unstable.tex}\medskip
    \input{../ch8_gnn/figures_stability/graph_dilation_stable.tex}    
    \caption{Stability of graph filters. We observe that, for small values of $\lambda$, the difference between $\lambda_{i}$ (in blue) and $\hlam_{i}$ (in red) is small, whereas for large $\lambda$ this becomes much larger. (top) When using a Lipschitz filter [cf. \eqref{eqn:lipschitzFilters}], we observe that for low frequencies, the response of the filter is very similar when instantiated on either $\lambda_{i}$ or $\hlam_{i}$; however, for large frequencies, the difference becomes much larger, and thus a small change in the eigenvalues, leads to a big change of the filter response in high frequencies. (bottom) In the case of integral Lipschitz filters [cf. \eqref{eqn:integralLipschitzFilters}], the effect on high frequencies is mitigated, by forcing the filter to be nearly constant at these frequencies, so that, when evaluated at eigenvalues that are far away, the filter response is still almost the same, guaranteeing stability.}
    \label{fig_graph_dilation}
\end{figure}

Suppose now that we are given a set of filter coefficients $\bbh$ and that we consider the filter $\bbH(\bbS)$ implemented on GSO $\bbS$ vis-\`a-vis the filter $\bbH(\hbS)$ implemented on another GSO $\hbS$. Given that the graph perturbation is inconsequential we would expect the filter differences to be inconsequential as well. Theorem \ref{thm:filterStabilityRelative} states that if the filters are integral Lipschitz this is true but if they are simply Lipschitz this need not be true. To understand why this happens we look at the differences between the spectra of $\bbS$ and $\hbS$.

Given that $\bbS$ and $\hbS$ are related by a scaling, they share the same set of eigenvectors and the scaling is translated to the eigenvalues. Thus, if $\bbS = \bbV\bbLam\bbV^{\Hr}$ is the eigenvector decomposition of $\bbS$ [cf. \eqref{eqn:eigendecomposition}], the eigenvector decomposition of $\hbS$ is
%
\begin{equation}\label{eqn:graphDilationEigenvalues}
   \hbS = \bbV \big[(1-\alpha)\bbLam\big]\bbV^{\Hr}.
\end{equation}
%
As per \eqref{eqn:graphDilationEigenvalues}, the eigenvalues of $\hbS$ are the eigenvalues of $\bbS$ scaled by a factor $(1-\alpha)$. Thus, the effect of the dilation in \eqref{eqn:graphDilation} on a filter with frequency response $h(\lam)$ is that instead of instantiating the response at eigenvalues $\lam_i$ we instantiate it at eigenvalues $(1-\alpha)\lam_i$. Consequently the response values that we expect to be $h(\lam_i)$ if the filter is run on $\bbS$ actually turn out to be $h((1-\alpha)\lam_i)$ if the filter is run on $\hbS$. This observation is the core argument in the proof of Theorem \ref{thm:filterStabilityRelative} and motivates three important observations that we discuss next.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\medskip \noindent {\bf Graph perturbations and filter perturbations.} Figure \ref{fig_graph_dilation} illustrates the effect of the dilation in \eqref{eqn:graphDilation} on a Lipschitz (top) and integral Lipschitz filter (bottom). The difference in the positions between eigenvalues is given by $\lam_i-\hlam_i = \alpha\lam_i$, and as such, depends on the value of the specific eigenvalue $\lambda_{i}$. For low graph frequencies $\lam_i$ the dilation results in a small perturbation of the eigenvalues. If the change in eigenvalues is small the change in the filter's response from $h(\lam_i)$ to $h(\hlam_i)$ is small for both filters. For large eigenvalues the difference $\lam_i-\hlam_i = \alpha\lam_i$ grows large. For Lipschitz filters a large difference in the arguments may translate into a large difference in the instantiated values of frequency responses $h(\lam_i)$ and $h(\hlam_i)$ since we can have
%
\begin{equation}\label{eqn_discussions_unstable}
   |h(\lam_i) - h(\hlam_i)| 
       \ \approx \ |\lam_i-\hlam_i| 
       \ =       \ \alpha\lam_i.
\end{equation}
%
This explains the filter's instability. A small graph perturbation may result in a large filter perturbation at high graph frequencies. For integral Lipschitz filters, on the other hand, changes in the frequency response must taper off as $\lam$ grows. Thus, even though there may be a large variation in the eigenvalues the instantiations of the frequency responses are close since we must have
%
\begin{equation}\label{eqn_discussions_stable}
   |h(\lam_i) - h(\hlam_i)| 
       \ \approx \ \frac{|\lam_i-\hlam_i|}{\lam_i} 
       \ =       \ \alpha.
\end{equation}
%
This explains the filter's stability. No matter how large the graph frequencies are, a small perturbation of the graph results in a small perturbation of the graph filter. Theorem \ref{thm:filterStabilityRelative} shows that this is true for arbitrary relative perturbations.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t]
    \centering
    \input{../ch8_gnn/figures_stability/high_frequency_feature.tex}      
    \caption{High frequency feature extraction. We illustrate two sharp filters designed to successfully extract high frequency features located at $\lambda_{N-1}$ and $\lambda_{N}$. However, when the graph is slightly perturbed, which results in large changes in high frequency eigenvalues, the designed filters are no longer able to extract these features, now located at $\hlam_{N-1}$ and $\hlam_{N}$, since they have moved out of the narrow pass band of the sharp filter.}
    \label{fig_high_frequency_feature}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\medskip \noindent {\bf Graph perturbations and feature identification.} There is an obvious cost we pay for the stability of integral Lipschitz filters: they are unable to discriminate high frequencies. The graph dilation example shows that this is not a limitation of the analysis. It is impossible to have a filter that is both stable and able to isolate high frequency features because small graph perturbations can result in large eigenvalue perturbations. This is a major drawback of linear graph filters in the extraction of features from graph signals. To illustrate this drawback suppose we have graph signals $\bbx_{1} = \bbv_N$ and $\bbx_2 = \bbv_{N-1}$ and we want to design graph filters to discriminate between the two. The graph frequency domain representation of these two signals on the graph $\bbS$ are shown in Figure \ref{fig_high_frequency_feature}. For us to discriminate between $\bbx_{1} = \bbv_N$ and $\bbx_2 = \bbv_{N-1}$ we need filters centered at frequencies $\lam_{N}$ and $\lam_{N-1}$. These filters must have sharp transitions so that the filter isolating $\bbx_1 = \bbv_{N}$ does not let the signal $\bbx_{2} = \bbv_{N-1}$ pass and, conversely, the filter isolating $\bbx_2 = \bbv_{N-1}$ does not let the signal $\bbx_{1} = \bbv_N$. Yet, if these filters are sharp in high frequencies, they will be unstable. More specifically, let $\hlam_{N} = (1-\alpha)\lambda_{N}$ be the eigenvalue associated to $\bbx_{1} = \bbv_{N}$ in the perturbed graph, and $\hlam_{N-1} = (1-\alpha)\lambda_{N-1}$ be the one associated to $\bbx_{2} = \bbv_{N-1}$. Now, since the filters were designed to be sharp around $\lambda_{N}$ and $\lambda_{N-1}$, but the perturbed eigenvalues $\hlam_{N}$ and $\hlam_{N-1}$ are far from these (at points where the filter response is virtually zero) the filter fails to adequately recover $\bbx_{1}$ and $\bbx_{2}$ in the perturbed graph. See Fig.~\ref{fig_high_frequency_feature} for an illustration of the high-frequency instability effect.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t]
\centering
\input{../ch8_gnn/figures_stability/relu_spectrum}      
\caption{Effect of pointwise nonlinearity. Let $\bbx = \bbv_{N}$ be the graph signal with a frequency response $\tbx$ given by $\tdx_{N}=1$ and $\tdx_{i} = 0$ for all $i=1,\ldots,N-1$. Signal $\bbx$ has a single nonzero value located at the highest frequency, making it impossible to be extracted with a stable linear filter. When applying a nonlinearity to this signal, we observe that nonzero frequency components arise throughout the spectrum, spilling the information contained in the highest frequency into lower frequencies. This facilitates the use of a bank of stable linear filters to successfully collect this information at lower frequencies. \blue{Add a second figure with relu output of eigenvalue placed at $\lam_{N-1}$.}}
\label{fig_relu_spectrum}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\medskip \noindent {\bf Pointwise nonlinearities.} So far, we have observed that stable filters require a flat response on high-frequencies, but that this inevitably prevents them from discriminating between features located at these frequencies. This illustrates an inherent, insurmountable limitation of linear information processing schemes. Neural networks introduce pointwise nonlinearities to the processing pipeline, as a computationally straightforward means of discriminating information at high frequencies. The basic effect of these nonlinearities is to cause a spillage of information throughout the frequency band, see Fig.~\ref{fig_relu_spectrum}. This spillage of information into lower frequencies allows for a stable filter to accurately discriminate between them, since information at lower frequencies does not get severely affected by perturbations. However, since the energy in lower frequencies is usually less than the energy still found at higher frequencies, and since it is also spread through a wide band of lower frequencies, the use of a bank of linear filters becomes a sensitive idea to better capture this spillage. Therefore, the use of banks of linear filters in combination with pointwise nonlinearities allows for information processing architectures that are able to capture high-frequency content in a stable fashion.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\medskip \noindent {\bf Frame of filter banks.} To get stability to perturbations, we require graph filters to be integral Lipschitz (Def.~\ref{eqn:integralLipschitzFilters}). To get enough discriminative power, we require a bank of filters, each one designed, or learned, to look after some specific feature. One further sensitive requirement, is that these filters cover up the whole frequency spectrum, that is, that they conform a \emph{frame}. Let $\{\bbH^{f}(\bbS)\}_{f=1,\ldots,F}$ be a filter bank, then it is called a frame, if it satisfies
% eqn
\begin{equation}
    A^{2} \| \bbx \|_{2}^{2} 
        \leq 
    \sum_{f=1}^{F} \| \bbH^{f}(\bbS) \bbx \|_{2}^{2} 
        \leq 
    B^{2} \| \bbx\|_{2}^{2}
\end{equation}
%
for some $0 < A \leq B < \infty$. The lower value $A$ controls how much a signal $\bbx$ is attenuated after being filtered, while the higher value $B$ determines the amplification. Typically, we would like $A$ to be bounded away from zero to avoid too much energy loss and, as we will see in the next section, we would like $B$ to be close to $1$ to improve stability of GNNs. Filter banks that are integral Lipschitz and conform a frame, can be typically obtained by using wavelets \cite{Hammond11-Wavelets, Shuman15-Wavelets}.






\blue{{\bf Eigenvector Normalization.} Why don't we just normalize the matrices? We can do this, but then what will happen is that filters can discriminate finely at low frequencies only because $h'(\lam)$ can be made very sharp close to 0. Lipshcitz filters can be made discriminative close to zero without blowing up the constant $C$}

==> ch8_sec15_recommendation_systems.tex <==
% !TEX root = root.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t] 
\def\myfactor{0.50}
\centering
\begin{minipage}{0.47\linewidth}\centering
\input{figures/hexagon_graph_signal}%\\ {\small (a)}
\end{minipage} \quad
\begin{minipage}{0.47\linewidth}\centering
\input{figures/hexagon_graph_signal_with_holes}%\\ {\small (b)}
\end{minipage}
\caption{Recommendation System. \blue{Write something.}}
\label{fig_ch1_reco_system_problem_formulation}
\end{figure}




\red{A recommendation system is made up of a set of customers or users denoted by $\ccalC$ and a set of products denoted by $\ccalM$. Customers have rated some products 

 with $x_{pi}$ denoting the rating given to product $p$ by user $i$. The goal is to predict the rating that user $i$ would give to product $p$ for products $p$ that $i$ has not yet rated. To that end, we consider sets of products that have been rated by pairs of users $(i,j)$ to define a user similarity network with edge weights
% 
\begin{align}\label{eqn_reco_systems_weights}
   w_{ij} = \frac{1}{|\ccalS_{ij}|}\sum_{p\in\ccalS_{ij}} (x_{pi}-\mu_{ij})(x_{pj}-\mu_{ij})
\end{align} 
%
where $\ccalS_{ij}$ is the set of products rated by both $i$ and $j$, and $\mu_{ij}:=(1/|\ccalS_{ij}|)\sum_{p\in \ccalS_{ij}}x_{pi}$. The weights $w_{ij}$ measure the correlation between users $i$ and $j$ based on their ratings to the same products. 

On the user similarity network, the collection of ratings to a product $p$ can be interpreted as a graph signal $\bbx_p$ where $[\bbx_p]_i = x_{pi}$ if $i \in \ccalS$ has rated $p$ and $0$ otherwise. 
This allows posing the recommendation problem for user $i$ as an ERM problem where the training set $\ccalT$ is built from graph signals associated with a subset of products $p$ for which $[\bbx_p]_i \neq 0$. Explicitly, the input samples are copies of $\bbx_p$ where the ratings given by user $i$ are ``zeroed-out'', and the output samples are the corresponding $x_{pi}$. The function $\bbPhi$ produces rating estimates $\hat{x}_{pi}$, and the optimal empirical classifier $\bbPhi^*$ is obtained by solving problem {\eqref{eqn_ch8_empirical_risk_minimization}} for the MSE loss $\ell(x_{pi},\hat{x}_{pi}) = (x_{pi}-\hat{x}_{pi})^2$. \red{L: Should I explain that the problem can also be solved for multiple users at a time?}


}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Recommendation Systems}\label{sec_ch8_reco_systems_stylized}

In a recommendation system we want to predict the ratings that customers or users would give to a certain product or item from the rating history of the product and the ratings that customers have given to similar products. Denote as $x_{ip}$ the rating that customer $i$ gives to product $p$. Typically, product $p$ has been rated by a subset of users which we denote $\ccalC_p$. From existing ratings we consider the sets of users $\ccalC_{pq}=\ccalC_{p} \cap \ccalC_{q}$ that have rated products $p$ and $q$ and compute similarity scores
% 
\begin{align}\label{eqn_reco_systems_weights}
   \sigma_{pq} = \frac{1}{|\ccalC_{pq}|}
                 \sum_{ i \in \ccalC_{pq}} 
                        (x_{ip}-\mu_{pq})(x_{iq}-\mu_{qp})
\end{align} 
%
where we have used the average ratings $\mu_{pq}=(1/|\ccalC_{pq}|)\sum_{i\in \ccalC_{pq}}x_{ip}$ and $\mu_{qp}=(1/|\ccalC_{pq}|)\sum_{i\in \ccalC_{pq}}x_{iq}$.

$w_{pq} = \sigma_{pq}/\sqrt{\sigma_{pp}\sigma_{qq}}$. Work with adjacency



\blue{\noindent Weiyu uses a normalization. Do we use it as well here?}

 \cite{HuangEtal18}.
 
 

The first step is to use the rating history of all products to compute a graph of product similarities, in which edges represent a similarity score between different products. This graph is assumed given to us and represented by a shift operator $\bbS$. The underlying assumption is that there exist an underlying set of true scores as shown in Figure \ref{fig_ch1_reco_system_problem_formulation} - (a), but that we only observe a subset of those scores as in Figure \ref{fig_ch1_reco_system_problem_formulation} - (b). The set of scores that are not observed can be estimated from the set of scores that have been observed. 

\paragraph{Training Set.} To build a training set for this problem we consider a collection of $U$ users and denote as $\bbx_i=[x_{i1},\ldots, x_{in}]^T$ the set of ratings that have been recorded for user $i$. In general, a user has rated a relatively small number of products, which we signify in Figure \ref{fig_ch1_reco_system_example_signals}- left with a large number of nodes for which $x_{ip}=0$. The indexes of the entries of $\bbx_i$ that are not zero are collected in the set $\ccalU_i:=\{p:x_{ip}\neq 0\}$. For each product that has been rated by a user, namely for each index $p\in\ccalU_i$, we define a vector $\bbx$ in which we set to zero the $p$th entry of $\bbx_i$. To write this formally, recall the definition of the canonical basis vector $\bbe_p$ which is all-zero except for the $p$th entry which is $[\bbe_p]_p=1$. Further define the matrix $\bbE_p = \bbI - \bbe_p\bbe_p^T$ which is an identity with the $p$th diagonal element set to zero. We can then isolate the rating of the $p$th product with the inner product $y = \bbe_p^T \bbx_i$ and remove this rating from $\bbx_i$ with the multiplication $\bbx = \bbE_p\bbx_i$. The pair $(\bbx,y)$ can be added to a training set to model the prediction of $y$ from a given set of ratings $\bbx$. Repeating this for all $p\in\ccalU_i$ and all users $i=1,\ldots, U$ we build the training set
% 
\begin{align}\label{eqn_ch8_reco_system_training_set}
   \ccalT = \big \{ (\bbx, y) \,:\, 
                    \bbx = \bbE_p\bbx_i,\ y = \bbe_p^T\bbx_i,  \text{\ for all\ } p\in\ccalU_i 
            \big \}_{i=1}^U .
\end{align}
%
The construction of an entry of the training set $\ccalT$ is illustrated in Figure \ref{fig_ch1_reco_system_example_signals}. In Figure \ref{fig_ch1_reco_system_example_signals}- left we have a rating signal $\bbx_i$ in which the nonzero entries are $\ccalU_i = \{2,3,4,8,9,10\}$. In Figure \ref{fig_ch1_reco_system_example_signals}- right we initialize $\bbx = \bbx_i$ and then set $x_3=0$. We further record the rating of product $3$ into the scalar value $y=x_{i3}$ and add the pair $(\bbx,y)$ to the training set. We repeat this for nodes 2, 4, 8, 9, and 10 and move on to consider the ratings of other users.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t] 
\def\myfactor{0.50}
\centering
\begin{minipage}{0.47\linewidth}\centering
\input{figures/hexagon_graph_signal_node_3_a} %\\ {\small (a)}
\end{minipage} \quad
\begin{minipage}{0.47\linewidth}\centering
\input{figures/hexagon_graph_signal_node_3_b}  %\\ {\small (b)}
\end{minipage} 
\caption{Training set for a recommendation system. The 6 shaded nodes in the left represent available ratings for a user $i$ with darker shadings representing higher ratings. Empty nodes are products that have not been rated by the user, which, as is typical, are a large fraction of all potential products. To build a training set we zero individual available ratings to model the prediction of this rating from the remaining available ones. In the figure in the right we have zeroed the rating of product 3 which we attempt to predict from the ratings of products 2, 4, 8, 9, and 10. Out all ratings of user $i$ we build 6 training set entries by sequentially zeroing each of the available ratings in the set $\ccalU_i = \{2,3,4,8,9,10\}$, [cf. \eqref{eqn_ch8_reco_system_training_set}].}\label{fig_ch1_reco_system_example_signals}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   M   A   I   N       M   A   T   T   E   R   %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\paragraph{Rating regression.} To make rating predictions we consider an arbitrary linear transform $\Phi(\bbx;\bbH) = \bbH \bbx$ with $\bbH\in\reals^{n\times n}$ as in \eqref{eqn_ch8_erm_linear}. This parametrizations predicts ratings for all nodes. If we are interested in isolating the rating of product $p$ we can do this by simply looking at the inner product $\bbe_p^T \Phi(\bbx; \bbH)$. This is, in particular, of interest when we consider training on the set $\ccalT$ defined by \eqref{eqn_ch8_reco_system_training_set} in which we have ratings of individual products recorded in the scalar $y$. Thus we consider losses of the form
% 
\begin{align}\label{eqn_ch8_reco_system_training_set_arbitrary_linear}
   \ell \big(\Phi(\bbx; \bbH), y \big) 
      \ = \ \frac{1}{2}\Big(\bbe_p^T \Phi(\bbx; \bbH) - y \Big)^2
      \ = \ \frac{1}{2}\Big(\bbe_p^T \bbH\bbx - y \Big)^2,
\end{align}
%
which we substitute in \eqref{eqn_ch8_erm_linear} and solve to find a rating prediction function $\Phi(\bbx;\bbH) = \bbH \bbx$.

Alternatively, we can use a linear graph filter $\Phi(\bbx;\bbh, \bbS) = \sum_{k=0}^\infty \bbS^k \bbx$ as in \eqref{eqn_ch8_erm_graph_filter}. This also produces ratings for all products but we can isolate the rating of product $p$ with the inner product $\bbe_p^T \Phi(\bbx;\bbh, \bbS)$. In particular, we can consider losses of the form
% 
\begin{align}\label{eqn_ch8_reco_system_training_set_graph_filter}
   \ell \big(\Phi(\bbx;\bbh, \bbS), y \big) 
       \ = \ \frac{1}{2}\Big(\bbe_p^T \Phi(\bbx;\bbh, \bbS) - y \Big)^2
       \ = \ \frac{1}{2}\bigg[\bbe_p^T \bigg(\sum_{k=0}^\infty h_k\bbS^k \bbx\bigg) - y \bigg]^2,
\end{align}
%
which we substitute in \eqref{eqn_ch8_erm_graph_filter} and solve to find a rating prediction graph filter $\Phi(\bbx;\bbh, \bbS) = \sum_{k=0}^\infty \bbS^k \bbx$. \green{In \eqref{eqn_ch8_reco_system_training_set_arbitrary_linear} and \eqref{eqn_ch8_reco_system_training_set_graph_filter} the vector $\bbe_p^T$ maps the output of the classifiers $\Phi(\bbx; \bbH)$ and $\Phi(\bbx;\bbh, \bbS)$ to the quantity of interest which is the rating at node $p$. We say that it is a readout function because it ``reads out'' the quantity of interest from the given classifier.}

\red{\paragraph{Rating classification.} User ratings are typically given as integers, which motivates a classification formulation. To make matters simplest suppose ratings are binary so that outputs are $y\in{-1,1}$ respectively signifying an inclination to buy the product or not. Inputs take on three values so that $\bbx_i \in\{-1,0,1\}^n$ with $x_{ip} = 0$ signify product $p$ has not been rated by user $i$.} \blue{It may be too much.}

\red{\paragraph{Readout functions.}} \blue{Linear and nonlinear readouts as a way of tying back to GNNs.}


\subsubsection{\red{Movie Rating Prediction}}

\blue{
Add some empirical results for predicting movie ratings with both models. The graph model will do better, hopefully.

This is a link to the movie recommendation results prepared by Luana and Fernando: {\tt https://docs.google.com/spreadsheets/d/1m6GS8NCfJFdNWqMufFIfU7B29gdBjNMjgcz5PGsQr2Y/edit?usp=sharing.} (Do not click on the link, it doesn't work. But copy and paste from the latex file. 

}

\blue{Some text to incorporate in a discussion motivating permutation invariance at the end of this section.} \red{After we have demonstrated the advangtage of graph filters a question arises: Why?} \green{In justifying \eqref{eqn_ch8_erm_graph_filter} as an alternative to \eqref{eqn_ch8_erm_linear}, we said that that the former leverages ``the fact that $\bbx$ is a graph signal.'' This statement begs the question of what exactly does it mean to exploit the fact that $\bbx$ is a graph signal. This question is more subtle than it seems because the graph filter in \eqref{eqn_ch8_erm_graph_filter} is a particular case of a linear function. It follows that for any given set of samples, the optimal solution of \eqref{eqn_ch8_erm_linear} has a smaller loss than the optimal solution of  \eqref{eqn_ch8_erm_graph_filter}. That is, we must have
% 
\begin{align}\label{eqn_ch8_linear_better_than_graph_filter}
   \bar\ell \big(\Phi(\xdot; \bbH) \big)  \leq \bar\ell \big(\Phi(\xdot; \bbh, \bbS) \big),
\end{align} 
%
because the solution of \eqref{eqn_ch8_erm_graph_filter} is a feasible choice for \eqref{eqn_ch8_erm_linear}. Our intuition, however, indicates that the opposite is true in some sense. The answer is, as it was the case in going from \eqref{eqn_ch8_empirical_risk_minimization} to \eqref{eqn_ch8_erm_learning}, that we do not observe all possible signals $\bbx_s$. It is true that \eqref{eqn_ch8_linear_better_than_graph_filter} holds when we consider the sample set. But when we test the loss for samples that have not been seen before, we expect the graph filter to perform better than an arbitrary linear map. This can be verified empirically but it is not difficult to see that the reason why this is bound to happen is due to the fact that graph filters exploit symmetries that are embedded in the structure of a graph signal. This brings us to the matter of permutation equivariance of graph filters which we tackle in the following section.}





\red{In Section \ref{sec_ch8_permutation_invariance_filters} we saw that graph filters are permutation equivariant. In Section \ref{sec_ch8_equivariance_and_symmetries} we explained that this property is critical in learning contexts as it exploits signal symmetries to generalize to unseen examples. The graph neural networks (GNNs) we introduce in this section extend graph filters while retaining permutation equivariance. They do so by using pointwise nonlinearities which are nonlinear functions that are applied independently to each component of a vector as we formally define next.}

To illustrate the problem of recommendation systems with a specific numerical example, we consider movie recommendation using the MovieLens-100k dataset \cite{harper16-movielens}. This dataset consists of 100,000 ratings given by 943 users to 1,682 movies, where each user has rated at least 10 movies. The movie ratings are integers between 1 and 5, and non-existing ratings are set to 0. The movie similarity network is built by computing Pearson correlations between pairs of movies as described in Section \red{X}. On this network, each user's rating vector $\bbx_i$ can be represented as a graph signal.

\begin{table}[t] 
\centering
\begin{tabular}{l|c|c|c} \hline
Parametrization          & $L$ & Hyperparameters & $\sigma$  \\ \hline
Linear param.    & -            & $n \times 1$ matrix  & -             \\
Graph filter     & -            & $F=64$, $K=5$                         & -              \\
FCNN             & 2            & $N_1=64$, $N_2=32$                    & ReLU          \\
G. perceptron & 1            & $K=5$                                 & ReLU          \\
G. perceptron & 2            & $K=5$                                 & ReLU           \\
GNN              & 1            & $F=64$, $K=5$                         & ReLU           \\
GNN              & 2            & $F_1=64$, $F_2=32$, $K=5$             & ReLU         \\ \hline
\end{tabular}
\caption{Hyperparameters of seven different parametrizations of $\Phi$ in \eqref{eqn_ch8_erm_learning}. The number of features, filter taps and hidden units are denoted $F$, $K$ and $N$ respectively. For multi-layer architectures, $F_\ell/N_\ell$ indicate the value of these hyperparameters at layer $\ell$.}
\label{tab:hyperparam}
\end{table}

Our goal is to predict the ratings to the movie ``Star Wars'' by solving the ERM problem in \eqref{eqn_ch8_erm_learning} with different parametrizations of $\Phi$. In order to do this, we follow the methodology in \red{X} to obtain 583 input-output pairs corresponding to users who have rated ``Star Wars''. This data is then split between 90\% for training (of which 10\% are used for validation) and 10\% for testing. 

Seven different parametrizations were considered: a simple linear parametrization; a graph filter \eqref{eqn_filter}; a fully connected neural network; a single-layer \eqref{eqn_ch8_perceptron_nonlinearity} and a multi-layer graph perceptron \eqref{eqn_ch8_gnn_recursion_single_feature_nonlinearity}; and a single-layer and a multi-layer GNN \eqref{eqn_ch8_gnn_recursion_nonlinearity_matrix}. Their hyperparameters are presented in Table \ref{tab:hyperparam}. All architectures were trained simultaneously by optimizing the L1 loss on the training set, using ADAM with learning rate $5 \times 10^{-3}$ and decay factors $0.9$ and $0.999$. The number of epochs and batch size were 40 and 5 respectively.

In Table \ref{tab:movie_results}, we report the average RMSE achieved by each parametrization for 10 random data splits. We observe that the linear graph filter obtains a much smaller error than the general linear parametrization, which highlights its superior ability in exploiting the structure of graph signals. The fact that the average RMSE of the fully connected neural network is worse than those of the GNNs, graph perceptrons and graph filter could be explained by the same reason, even if the fully connected neural network improves upon the linear transformation due to the addition of nonlinearities. The graph perceptrons are not better than the graph filter and showcase similar RMSEs in both the single and multi-layer case. On the other hand, the addition of multiple features in the single-layer and multi-layer GNNs provide sensible improvements, with the 2-layer GNN performing better than all other architectures.

\begin{table}[t]
\centering
\begin{tabular}{l|c} \hline
Parametrization        & RMSE   \\ \hline
Linear parametrization & 1.8527 \\
Graph filter           & 0.8025 \\
FCNN                   & 0.9897 \\
Graph perceptron, $L=1$ & 0.8061 \\
Graph perceptron, $L=2$ & 0.8067 \\
GNN, $L=1$              & 0.7930 \\
GNN, $L=2$              & 0.7663 \\ \hline
\end{tabular}
\caption{Average RMSE achieved by each parametrization in 10 random data splits for the movie ``Star Wars''.}
\label{tab:movie_results}
\end{table}












==> ch8_sec15_recommendation_systems_old.tex <==
% !TEX root = ../compile_all_book/gsp.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t] 
\def\myfactor{0.70}
\centering
\begin{minipage}{0.47\linewidth}\centering
\input{../ch8_gnn/figures/hexagon_graph_signal}%\\ {\small (a)}
\end{minipage} \quad
\begin{minipage}{0.47\linewidth}\centering
\input{../ch8_gnn/figures/hexagon_graph_signal_with_holes}%\\ {\small (b)}
\end{minipage}
\caption{Recommendation System. \blue{Write something.}}
\label{fig_ch1_reco_system_problem_formulation}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Recommendation Systems}\label{sec_ch8_reco_systems_stylized}

In a recommendation system we want to predict the rating that a user would give to a certain product from the observed history of the agent and the ratings that other users have given to this product. The first step is to use the history of all agents to compute a graph of agent similarities, in which edges represent a similarity score between different agents. This graph is assumed given to us and represented by a shift operator $\bbS$. The underlying assumption is that there exist an underlying set of true scores as shown in Figure \ref{fig_ch1_reco_system_problem_formulation} - (a), but that we only observe a subset of those scores as in Figure \ref{fig_ch1_reco_system_problem_formulation} - (b). The set of scores that are not observed can be estimated from the set of scores that have been observed. 

\paragraph{Training Set.} To build a training set for this problem we consider a collection of $P$ products and denote as $\bbx_p=[x_{p1},\ldots, x_{pn}]^T$ the set of ratings that have been recorded for product $p$. In general, a relatively small number of users have rated a product, which we signify in Figure \ref{fig_ch1_reco_system_example_signals}- left with a large number of nodes for which $x_{pi}=0$. The indexes of the entries of $\bbx_p$ that are not zero are collected in the set $\ccalU_p:=\{i:x_{pi}=0\}$. For each user that has rated a product, namely for each index $i\in\ccalU_p$, we define a vector $\bbx$ in which we set to zero the $i$th entry of $\bbx_p$. To write this formally, recall the definition of the canonical basis vector $\bbe_i$ which is all-zero except for the $i$th entry which is $[\bbe_i]_i=1$. Further define the matrix $\bbE_i = \bbI - \bbe_i\bbe_i^T$ which is an identity with the $i$th diagonal element set to zero. We can then isolate the rating of the $i$th user with the inner product $y = \bbe_i^T \bbx_p$ and remove this rating from $\bbx_p$ with the multiplication $\bbx = \bbE_i\bbx_p$. The pair $(\bbx,y)$ can be added to a training set to model the prediction of $y$ from a given set of ratings $\bbx$. Repeating this for all $i\in\ccalU_p$ and all products $p=1,\ldots, P$ we build the training set
% 
\begin{align}\label{eqn_ch8_reco_system_training_set}
   \ccalT = \big \{ (\bbx, y) \,:\, 
                    \bbx = \bbE_i\bbx_p,\ y = \bbe_i^T\bbx_p,  \text{\ for all\ } i\in\ccalU_p 
            \big \}_{p=1}^P .
\end{align}
%
The construction of an entry of the training set $\ccalT$ is illustrated in Figure \ref{fig_ch1_reco_system_example_signals}. In Figure \ref{fig_ch1_reco_system_example_signals}- left we have a rating signal $\bbx_p$ in which the nonzero entries are $\ccalU_p = \{2,3,4,8,9,10\}$. In Figure \ref{fig_ch1_reco_system_example_signals}- right we initialize $\bbx = \bbx_p$ and then set $x_3=0$. We further record the rating of user $3$ into the scalar value $y=x_{p3}$ and add the pair $(\bbx,y)$ to the training set. We repeat this for nodes 2, 4, 8, 9, and 10 and move on to consider the ratings of other products.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t] 
\def\myfactor{0.70}
\centering
\begin{minipage}{0.47\linewidth}\centering
\input{../ch8_gnn/figures/hexagon_graph_signal_node_3_a} %\\ {\small (a)}
\end{minipage} \quad
\begin{minipage}{0.47\linewidth}\centering
\input{../ch8_gnn/figures/hexagon_graph_signal_node_3_b}  %\\ {\small (b)}
\end{minipage} 
\caption{Training set for a recommendation system. The 6 shaded nodes in the left represent available ratings for a product $p$ with darker shadings representing higher ratings. Empty nodes are users that have not rated the product, which, as is typical, are a large fraction of all potential clients. To build a training set we zero individual available ratings to model the prediction of this rating from the remaining available ones. In the figure in the right we have zeroed the rating of agent 3 which we attempt to predict from the ratings of users 2, 4, 8, 9, and 10. Out all ratings of product $p$ we build 6 training set entries by sequentially zeroing each of the available ratings in the set $\ccalU_p = \{2,3,4,8,9,10\}$, [cf. \eqref{eqn_ch8_reco_system_training_set}].}\label{fig_ch1_reco_system_example_signals}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   M   A   I   N       M   A   T   T   E   R   %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\paragraph{Rating regression.} To make rating predictions we consider an arbitrary linear transform $\Phi(\bbx;\bbH) = \bbH \bbx$ with $\bbH\in\reals^{n\times n}$ as in \eqref{eqn_ch8_erm_linear}. This parametrizations predicts ratings for all nodes. If we are interested in isolating the rating of user $i$ we can do this by simply looking at the inner product $\bbe_i^T \Phi(\bbx; \bbH)$. This is, in particular, of interest when we consider training on the set $\ccalT$ defined by \eqref{eqn_ch8_reco_system_training_set} in which we have ratings of individual users recorded in the scalar $y$. Thus we consider losses of the form
% 
\begin{align}\label{eqn_ch8_reco_system_training_set_arbitrary_linear}
   \ell \big(\Phi(\bbx; \bbH), y \big) 
      \ = \ \frac{1}{2}\Big(\bbe_i^T \Phi(\bbx; \bbH) - y \Big)^2
      \ = \ \frac{1}{2}\Big(\bbe_i^T \bbH\bbx - y \Big)^2,
\end{align}
%
which we substitute in \eqref{eqn_ch8_erm_linear} and solve to find a rating prediction function $\Phi(\bbx;\bbH) = \bbH \bbx$.

Alternatively, we can use a linear graph filter $\Phi(\bbx;\bbh, \bbS) = \sum_{k=0}^\infty \bbS^k \bbx$ as in \eqref{eqn_ch8_erm_graph_filter}. This also produces ratings for all users but we can isolate the rating of user $i$ with the inner product $\bbe_i^T \Phi(\bbx;\bbh, \bbS)$. In particular, we can consider losses of the form
% 
\begin{align}\label{eqn_ch8_reco_system_training_set_graph_filter}
   \ell \big(\Phi(\bbx;\bbh, \bbS), y \big) 
       \ = \ \frac{1}{2}\Big(\bbe_i^T \Phi(\bbx;\bbh, \bbS) - y \Big)^2
       \ = \ \frac{1}{2}\bigg[\bbe_i^T \bigg(\sum_{k=0}^\infty h_k\bbS^k \bbx\bigg) - y \bigg]^2,
\end{align}
%
which we substitute in \eqref{eqn_ch8_erm_graph_filter} and solve to find a rating prediction graph filter $\Phi(\bbx;\bbh, \bbS) = \sum_{k=0}^\infty \bbS^k \bbx$. \green{In \eqref{eqn_ch8_reco_system_training_set_arbitrary_linear} and \eqref{eqn_ch8_reco_system_training_set_graph_filter} the vector $\bbe_i^T$ maps the output of the classifiers $\Phi(\bbx; \bbH)$ and $\Phi(\bbx;\bbh, \bbS)$ to the quantity of interest which is the rating at node $i$. We say that it is a readout function because it ``reads out'' the quantity of interest from the given classifier.}

\red{\paragraph{Rating classification.} User ratings are typically given as integers, which motivates a classification formulation. To make matters simplest suppose ratings are binary so that outputs are $y\in{-1,1}$ respectively signifying an inclination to buy the product or not. Inputs take on three values so that $\bbx_p \in\{-1,0,1\}^n$ with $x_{pi} = 0$ signifying product $p$ has not been rated by user $i$.} \blue{It may be too much.}

\red{\paragraph{Readout functions.}} \blue{Linear and nonlinear readouts as a way of tying back to GNNs.}


\subsubsection{\red{Movie Rating Prediction}}

\blue{
\bi Add some empirical results for predicting movie ratings with both models. The graph model will do better, hopefully.\ei

%\bi This is a link to the movie recommendation results prepared by Luana and Fernando: {\tt https://docs.google.com/spreadsheets/d/1m6GS8NCfJFdNWqMufFIfU7B29gdBjNMjgcz5PGsQr2Y/edit?usp=sharing.} (Do not click on the link, it doesn't work. But copy and paste from the latex file. \ei

}

\blue{Some text to incorporate in a discussion motivating permutation invariance at the end of this section.} \red{After we have demonstrated the advangtage of graph filters a question arises: Why?} \green{In justifying \eqref{eqn_ch8_erm_graph_filter} as an alternative to \eqref{eqn_ch8_erm_linear}, we said that that the former leverages ``the fact that $\bbx$ is a graph signal.'' This statement begs the question of what exactly does it mean to exploit the fact that $\bbx$ is a graph signal. This question is more subtle than it seems because the graph filter in \eqref{eqn_ch8_erm_graph_filter} is a particular case of a linear function. It follows that for any given set of samples, the optimal solution of \eqref{eqn_ch8_erm_linear} has a smaller loss than the optimal solution of  \eqref{eqn_ch8_erm_graph_filter}. That is, we must have
% 
\begin{align}\label{eqn_ch8_linear_better_than_graph_filter}
   \bar\ell \big(\Phi(\xdot; \bbH) \big)  \leq \bar\ell \big(\Phi(\xdot; \bbh, \bbS) \big),
\end{align} 
%
because the solution of \eqref{eqn_ch8_erm_graph_filter} is a feasible choice for \eqref{eqn_ch8_erm_linear}. Our intuition, however, indicates that the opposite is true in some sense. The answer is, as it was the case in going from \eqref{eqn_ch8_empirical_risk_minimization} to \eqref{eqn_ch8_erm_learning}, that we do not observe all possible signals $\bbx_s$. It is true that \eqref{eqn_ch8_linear_better_than_graph_filter} holds when we consider the sample set. But when we test the loss for samples that have not been seen before, we expect the graph filter to perform better than an arbitrary linear map. This can be verified empirically but it is not difficult to see that the reason why this is bound to happen is due to the fact that graph filters exploit symmetries that are embedded in the structure of a graph signal. This brings us to the matter of permutation equivariance of graph filters which we tackle in the following section.}





\red{In Section \ref{sec_ch8_permutation_invariance_filters} we saw that graph filters are permutation equivariant. In Section \ref{sec_ch8_equivariance_and_symmetries} we explained that this property is critical in learning contexts as it exploits signal symmetries to generalize to unseen examples. The graph neural networks (GNNs) we introduce in this section extend graph filters while retaining permutation equivariance. They do so by using pointwise nonlinearities which are nonlinear functions that are applied independently to each component of a vector as we formally define next.}

















==> figures/signal_color_code.tex <==
\tikzstyle{empty node} = [ circle, 
                     draw = black,
                     text = black, 
                     minimum size = 1.0*\unit]
%
\tikzstyle{node value a} = [ empty node, 
                     fill = blue!90,
                     draw = blue!90,
                     text = white]
%
\tikzstyle{node value b} = [ empty node, 
                     fill = blue!55,
                     draw = blue!55,
                     text = white]
%
\tikzstyle{node value c} = [ empty node, 
                     fill = blue!35,
                     draw = blue!35,
                     text = white]
%
\tikzstyle{node value d} = [ empty node, 
                     fill = blue!15,
                     draw = blue!15,
                     text = white]
%
\tikzstyle{faded node} = [ empty node, 
                     draw = black!30,
                     text = black!30]
%

